Consistent Counterfactuals for Deep Models

Counterfactual examples are one of the most commonly-cited methods for explaining the predictions of machine learning models in key areas such as finance and medical diagnosis. Counterfactuals are often discussed under the assumption that the model on which they will be used is static, but in deployment models may be periodically retrained or fine-tuned. This paper studies the consistency of model prediction on counterfactual examples in deep networks under small changes to initial training conditions, such as weight initialization and leave-one-out variations in data, as often occurs during model deployment. We demonstrate experimentally that counterfactual examples for deep models are often inconsistent across such small changes, and that increasing the cost of the counterfactual, a stability-enhancing mitigation suggested by prior work in the context of simpler models, is not a reliable heuristic in deep networks. Rather, our analysis shows that a model's local Lipschitz continuity around the counterfactual is key to its consistency across related models. To this end, we propose Stable Neighbor Search as a way to generate more consistent counterfactual explanations, and illustrate the effectiveness of this approach on several benchmark datasets.

==> 06_Discussion.tex <==
\section{Discussion}\label{sec:discussion}

==> 08_Others.tex <==
% !TEX ROOT=./neurips_2021.tex
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}, in Section ~\ref{sec:limitations}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}, in Section ~\ref{sec:limitations}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}, either fully within the theorem statement (e.g. Theorem~\ref{theorem:cost-in-deep-models}, Theorem~\ref{theorem:lowerbound-of-gradient-norm}), or directly prior in the section, as in Theorem ~\ref{theorem:loss-and-lipschitz} in Section~\ref{sec:lipschitz}. 
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} In Section ~\ref{appendix:proofs} in the Appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} in Section ~\ref{appendix:experiment-details}.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} in Section ~\ref{appendix:error-bars}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} in Section ~\ref{sec:evaluation} in paragraph entitled "Retraining Controls".
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} in Section~\ref{sec:evaluation} in paragraph entitled "Datasets".
  \item Did you mention the license of the assets?
    \answerYes{} in Section~\ref{appendix:experiment-details-datasets}.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> RNS.tex <==
% !TEX ROOT=./neurips_2021.tex

The results from the previous section suggest that counterfactuals from more locally-Lipschitz regions of the model will be more consistent across related models.
\emph{Stable Neighbor Search} leverages this intuition to find consistent counterfactuals by searching for those with a low local Lipschitz constant. We can find such points with
%This intuition is formalized by 
the objective in Equation~\ref{Eq:find_small_K}, which assumes a given counterfactual point $\xvec$.
\begin{align}\label{Eq:find_small_K}
    \xvec_c = \arg\min_{\xvec' \in B(\xvec, \delta)} K(\xvec', \epsilon)
    \quad
    \text{such that}\ 
    F(\xvec_c; \theta) = F(\xvec; \theta)
\end{align} 
Leveraging a well-known relationship between the dual norm of the gradient and a function's local Lipschitz constant~\cite{Paul}, we can rephrase this objective as shown in Equation~\ref{Eq:find_robust_neighbor}. 
Note that we assume $\ell_2$ norms throughout, so the dual leaves the norm unchanged.
In the rest of this section, we assume for the sake of clarity that $F$ is a binary classifier with a single-logit output; the results are readily extended to multi-logit outputs by optimizing over the maximal logit at $\xvec$.
\begin{align}\label{Eq:find_robust_neighbor}
    \xvec_c = \arg\min_{\xvec' \in B(\xvec, \delta)}\ \max_{\myhat{\xvec} \in B(\xvec', \epsilon)} \{||\nabla f(\myhat{\xvec}; \theta)||_2\}
    \quad
    \text{such that}\ 
    F(\xvec_c; \theta) = F(\xvec; \theta)
\end{align} 
While Equation~(\ref{Eq:find_robust_neighbor}) provides an objective that uses only primitives that are readily available in most neural network frameworks, it is not a practical solution for two principle reasons: \emph{1)} solving the inner objective using gradient descent requires second-order derivatives of $f$, which are always $\boldsymbol{0}$ in a ReLU network; and \emph{2)} the bilevel optimization problem is computationally prohibitive. 
In the following, we discuss a sequence of relaxations to Eq.~(\ref{Eq:find_robust_neighbor}) that address these challenges.

\paragraph{Avoiding vacuous second-order derivatives.} 
To solve the first problem, we need a substitution for $||\nabla f(\myhat{\xvec}, \theta)||_2$ that will provide useful gradients for the outer minimization. 
Ghorbani et al.~\cite{ghorbani2019interpretation} show that replacing ReLU activations with a related twice-differentiable activation, such as Softplus, can be a fruitful approach. 
However, this can also lead to a model with a substantially different decision surface, which complicates enforcing the equality constraint over $F$ during optimization.
Instead, we introduce a parameter $t$ over which we can take the derivative, in place of $\myhat{x}$, allowing the subsequent derivative with respect to $\xvec'$ to succeed.
Proposition~\ref{theorem:lowerbound-of-gradient-norm} shows that such a $t$ exists, and how to construct it.

\begin{proposition}\label{theorem:lowerbound-of-gradient-norm}
    Let $h$ be a differentiable, real-valued function in $\mathbb{R}^d$.
    Then for $\xvec \in \mathbb{R}^d$:
    \[
    \forall\xvec' \in B_2(\xvec, \epsilon).
    ||\nabla_{\xvec'} h(\xvec')||_2 \ge (||\xvec||_2+\epsilon)^{-1} \cdot |\nabla_t h(t\xvec')|_{t=1}|
    \]
\end{proposition}

Proposition~\ref{theorem:lowerbound-of-gradient-norm} allows us to relax Eq.~\ref{Eq:find_robust_neighbor} by maximizing a differentiable lower-bound of the gradient norm rather than the gradient norm itself.
Noting that the constant factor $||\xvec||_2+\epsilon$ is irrelevant to the desired optimization problem, Equation~\ref{Eq:find_robust_neighbor-challenge-one} below updates the objective accordingly. 
\begin{align}\label{Eq:find_robust_neighbor-challenge-one}
    \xvec_c = \arg\min_{\xvec' \in B(\xvec, \delta)}\ \max_{\myhat{\xvec} \in B(\xvec', \epsilon)} \{|\nabla_t f(t\myhat{\xvec}; \theta)|_{t=1}|\}
    \quad
    \text{such that}\ 
    F(\xvec_c, \theta) = F(\xvec;\theta)
\end{align}

\paragraph{Efficient bilevel approximation.} 
The second challenge mentioned above is the computational feasibility of solving the inner maximization. 
There are numerous techniques aimed at similar problems~\cite{Goodfellow2015ExplainingAH, madry2018towards}, including the sometimes simple-but-effective approach of returning the empirical maximum over a random sample of points in the targeted region~\cite{hill2020wrongfully}.
We take a more targeted approach, maximizing the gradient along a linear path from $\xvec'$ to the boundary of $B(\xvec', \epsilon)$.
This allows us to approximate the maximization using line search, simplifying the computation of the bilevel optimization greatly.
Figure~\ref{fig:illustration-circle} provides an intuitive illustration.
Eq.~\ref{Eq:find_robust_neighbor-challenge-two} shows the objective updated accordingly.
\begin{align}\label{Eq:find_robust_neighbor-challenge-two}
    \xvec_c = \arg\min_{\xvec' \in B(\xvec, \delta)}\ \max_{t \in [a,1]} \{|\nabla_t f(t\myhat{\xvec}; \theta)|\}
    \ 
    \text{such that}\ 
    F(\xvec_c; \theta) = F(\xvec; \theta),
    a = \epsilon||\xvec'||^{-1}
\end{align}
As we show in Section~\ref{sec:evaluation}, this approach works well in practice.

\paragraph{Finding a valid solution.} 
The discussion so far has shown how to relax the objective while still promoting solutions that reside in flatter regions of the decision surface.
In practice, we must also avoid violating the equality constraint which ensures that the solution will remain a counterfactual.
To discourage this, we add a term to encourage the network to remain confident about the current solution, which has the effect of controlling the gradient norm as $t\rightarrow 1$.
This is motivated by our empirical observation that when a network becomes confident at an early stage when $t \ll 1$, its output tends to stabilize later when $t\rightarrow 1$.
A visual illustration is shown in Fig.~\ref{fig:illustration-curve}. 
As we plot the network's output against $t$ for a starting point $\xvec$, it usually has a large slope, like curve $A$, when $t \rightarrow 1$, as depicted by the shaded area in light gray.
We expect that a counterfactual input $\xvec_c$, where the curve of $f(t\xvec_c, \theta)$ against $t$ has flattened tail and high confidence, to obey the optimization constraint.
Curve B is an example where the slope occurs sooner (before the dark shaded region), and so it has smaller gradient norm as $t \rightarrow 1$ (the light shaded region). 
The quantity obtained by integrating $-|f(t\xvec'; \theta)|$ over $[0,1]$ encourages this behavior when added to the minimization objective.

\paragraph{Final objective.}
Putting everything together, Figure~\ref{def:SNS} shows our objective for \emph{Stable Neighbor Search} (SNS), which finds a more stable counterfactual example nearby one that is given.

% As we notice that $f(\zvec') = f(r(t, \zvec'))|_{t=1}$ where $r(t, \zvec') = t\zvec'$, we find that by encouraging the network's output confidence on the intermediate points $t\zvec', 0\leq t<1$, it also helps to decrease the gradient norm $|\nabla_t f_i(r(t, \zvec^{\dagger}))|$ as $t\rightarrow 1$ because our emprirical evidence shows that when a network becomes fairly confident at an early stage when $t \ll 1$, its output tends to stabilize later when $t\rightarrow 1$. 

\begin{definition}[Stable Neighbor Search (SNS)]\label{def:SNS}
Given a starting counterfactual $\xvec$ for a network $F(\xvec, \theta)$, its \emph{stable neighbor} $\xvec_c$ of radius $\epsilon$ is the solution to the following objective: 
\[
    \arg\min_{\xvec' \in B(\xvec, \delta)}\ \max_{t \in [a,1]} \{|\nabla_t f(t\myhat{\xvec}; \theta)|\}- \int^1_{0} |f(t\xvec'; \theta)| \, dt
\quad \text{where} \quad
a = \epsilon||\xvec'||_2^{-1}
\]
\end{definition}

We discuss the choice of $\epsilon$, which controls the size of the stable region around $\xvec_c$, in Sec.~\ref{sec:evaluation}.
To implement Def.~\ref{sec:sns}, the integral is replaced by a summation over a grid of points of a specified resolution, which controls the quality of the final approximation. 

% \paragraph{Summary.} In this subsection, we propose SNS as a method to find consistent counterfactuals. To this end, we begin with finding points that minimize the low local Lipschitz constants in their neighborhood. We identify two challenges when directing solving the initial objective (Eq.(\ref{Eq:find_robust_neighbor})) and we discuss the techniques used to solve them respectively. Finally, we introduce the definiton of SNS in Eq.~(\ref{Eq:SNS}).
%In Stable Neighbor Search, we aim to find consistently predicted counterfactuals by searching for points with low Lipschitz constants in their neighborhood. 
% Stable Neighbor Search can work on top of any counterfactual search method: given a counterfactual, SNS searches for a nearby point with a low Lipschitz constant. Thus, we formulate the objective of SNS as follows: given an input $\xvec$, a classifier $F(\xvec;\theta)$ and a (potentially inconsistent) counterfactual example $\zvec$ generated by some counterfactual generation method, we want to find a nearby consistently predicted counterfactual $\xvec_c$ by searching for a point where the model's loss has a low a Lipschitz constant in its neighborhood. 

% Motivated by Theorem~\ref{theorem:loss-and-lipschitz}, in this subsection we discuss our approach to finding consistent counterfactual examples in deep models. Given an input $\xvec$, a classifier $F(\xvec;\theta)$ and its counterfactual but potentially inconsistent counterfactual example $\zvec$ found by methods discussed in Sec.~\ref{sec:invalidation}, the local Lipschitz Constant $K$ in a neighborhood $B(\zvec, \epsilon)$ for the classifier's logit output $f_i, i = F(\zvec;\theta)$ is given by the following equation: $K = \max_{\zvec' \in B(\zvec, \epsilon)} ||\nabla_\zvec' f_i(\zvec')||_q$~\cite{} where the dual norm $q=2$ for the $\ell_2$ norm used in this paper. To find a new counterfactual example $\xvec_c$ with small local Lipschitz Constant, we consider the following objective
% \begin{align}\label{Eq:find_robust_neighbor}
%     \xvec_c = \arg\min_{\zvec' \in B(\zvec, \delta)} \max_{\zvec^{\dagger} \in B(\zvec', \epsilon)} ||\nabla f_i(\zvec^{\dagger})||, \quad s.t. F(\xvec_c) = F(\zvec)
% \end{align}
% where the inner-max computes the local Lipschitz Constant and the outter-min finds the counterfactual example with the smallest local Lipschitz Constant within a user-defined neighborhood $B(\zvec, \delta)$. Eq.~(\ref{Eq:find_robust_neighbor}) provides a theoretical solution to find consistent counterfactual examples but is not a practical solution because of the following \textbf{challenges}: 1) the second-order derivatives required to solve Eq.~(\ref{Eq:find_robust_neighbor}) are always zero vectors in piece-wise linear networks; and 2) the min-max optimization is computationally expensive. We now discuss several relaxations for Eq.~(\ref{Eq:find_robust_neighbor}) to solve these two challenges. We begin with Theorem~\ref{theorem:lowerbound-of-gradient-norm}.

% \begin{theorem}\label{theorem:lowerbound-of-gradient-norm}
%     Suppose $h: \mathbb{R}^d \rightarrow \mathbb{R}$ is a differentiable and real-valued function in $\mathbb{R}^d$, $\forall \xvec' \in B(\xvec, \epsilon)$, $||\nabla_{\xvec'}h(\xvec')|| \geq C \cdot |\nabla_t h(r(t, \xvec'))|_{t=1}|$ where $C = 1/(||\xvec||+\epsilon)$ and $r(t, \xvec')$ is a linear path from a zero vector baseline input to the target input $\xvec'$ such that $r(t, \xvec') = t\xvec'$.
% \end{theorem}

% \begin{figure}[t]
%     \centering
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{images/circle.jpg}
%         \caption{placeholder}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{images/circle.jpg}
%         \caption{}
%         \label{fig:illustration-circle}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \includegraphics[width=\textwidth]{images/curve.jpg}
%         \caption{}
%         \label{fig:illustration-curve}
%      \end{subfigure}
%     \caption{TODO}
%  \end{figure}

% \paragraph{Solution to Challenge One.} Theorem~\ref{theorem:lowerbound-of-gradient-norm} describes a lower-bound of the gradient norm; therefore, it can be used to lower-bound the inner-max of Eq.~(\ref{Eq:find_robust_neighbor}). Because the derivative is w.r.t $t$ instead of the input, we only need the first-order derivatives w.r.t the input to perform gradient descent. We now give some intuitions about how the theorem is developed: we look for a way to capture the change of the function's output gradient w.r.t the input without actually computing the gradient because we would like to save it for running the optimization in Eq.~(\ref{Eq:find_robust_neighbor}). Such method is found in the definition of Integrated Gradient (IG)~\cite{}, a gradient-based explanation approach originally proposed to measure the feature importance by attributing a function's output $h(\xvec)$ over each input feature. IG aggregates the gradient of the network's output w.r.t. all points over a linear path $r(t; \xvec, \xvec_b)$ from a baseline input $\xvec_b$ to the input of interest $\xvec$ where $r(t; \xvec, \xvec_b) = \xvec_b + (\xvec - \xvec_b)t, t \in [0, 1]$. Therefore, by using the chain rule we find that $\nabla_t f(r(t; \xvec, \xvec_b)) = \langle \xvec - \xvec_b, \nabla_\xvec h(\xvec) \rangle$, which provides a way to capture the change of $\nabla_\xvec h(\xvec)$ through the inner product and without actually computing the derivative. The full proof of Theorem~\ref{theorem:lowerbound-of-gradient-norm} is provided in \textcolor{blue}{Appendix}. By using Theorem~\ref{theorem:lowerbound-of-gradient-norm}, we modify Eq.~(\ref{Eq:find_robust_neighbor}) as follows:

% \begin{align}\label{Eq:find_robust_neighbor-challenge-one}
%     \xvec_c = \arg\min_{\zvec' \in B(\zvec, \delta)} \max_{\zvec^{\dagger} \in B(\zvec', \epsilon)} |\nabla_t f_i(r(t, \zvec^{\dagger}))|_{t=1}|, \quad s.t. F(\xvec_c) = F(\zvec), \quad r(t, \zvec^{\dagger}) = t\zvec^{\dagger}
% \end{align}

% \paragraph{Solution to Challenge Two.} Approximating the inner-max has been the topic for many ML researches, e.g. adversarial training~\cite{}. The simplest approximation is to use one or randomly sampled points in the neighborhood $B(\zvec', \epsilon)$ to lower-bound the actual inner-max, which has been shown to be effective and promising in training empirically robust networks~\cite{}. As Theorem~\ref{theorem:lowerbound-of-gradient-norm} suggests that the gradient norm can be bounded by computing derivatives at the end ($t=1$) of a linear path $r(t;\xvec')$, we use all the points on the line segment within $B(\zvec', \epsilon)$ to approximate the inner-max as follows:

% \begin{align}\label{Eq:find_robust_neighbor-challenge-two}
%     \xvec_c = \arg\min_{\zvec' \in B(\zvec, \delta)} \max_{t \in [a,1]} |\nabla_t f_i(r(t, \zvec'))|, \quad s.t. F(\xvec_c) = F(\zvec),\quad r(t, \zvec') = t\zvec'
% \end{align}
% where $a=\epsilon/||\zvec'||$ and we show the corresponding visual illustration in Fig.~\ref{fig:illustration-circle}. That is, we approximate the maximum gradient $\max_{\zvec^{\dagger} \in B(\zvec', \epsilon)} |\nabla_t f_i(r(t, \zvec^{\dagger}))|_{t=1}|$ only using points on the line segment which corresponding to $t = [a, 1]$. In practice, the proposed line segment approximation is effective and we will empirically validate this in Sec.~\ref{sec:evaluation}.

% \paragraph{Implementation.} We find implementing Eq.~(\ref{Eq:find_robust_neighbor-challenge-two}) in practice may lead to trivial solution because the network can cheat by decreasing the $f_i(r(t, \zvec')$ for all points for $t\in[0,1]$ to minimize $|\nabla_t f_i(r(t, \zvec'))|$, which makes the optimization to stop early as we will always end up with violating the constraint $F(\xvec_c) = F(\zvec)$. As we plot the output of $f_i(r(t, \zvec'))$ against $t$ in Fig.~\ref{fig:illustration-curve}, we discover that before the optimization of Eq.~(\ref{Eq:find_robust_neighbor-challenge-two}), we usually have large slopes when $t \rightarrow 1$ (the shaded area in light gray), e.g. curve A.  We expect a counterfactual input $\xvec_c$ where the curve of $f_i(r(t, \xvec_c))$ against $t$ has flattened tail in the light shaded region with high confidence to ensure $F(\xvec_c) = F(\zvec)$, e.g. curve B. Therefore, we encourage the network to increase its output of $f_i(r(t, \zvec'))$ even at an early stage shaded in dark gray in Fig.~\ref{fig:illustration-curve} when $t<1$. Finally, we formally introduce the proposed approach in finding consistent counterfactual example, \emph{Robust Neighbor Search}. We will later discuss the choice of hyper-parameters and the implementation details in Sect.~\ref{sec:evaluation}.

% \begin{definition}[Robust Neighbor Search (SNS)]\label{def:SNS}
% Given a data point $\xvec$ and a counterfactual input $\zvec$ for a network $F(\xvec)$, a more consistent counterfactual example $\xvec_c$ can be found by optimizing the following objective:
% \begin{align}
%     &\xvec_c = \arg\min_{\zvec' \in B(\zvec, \delta)} \left[ \max_{t \in [a,1]} |\nabla_t f_i(r(t, \zvec'))| - \sum_{t\in[0,1]} f_i(r(t, \zvec')) \right]\\
%     &s.t. F(\xvec_c) = F(\zvec)
%     \label{Eq:find_robust_neighbor}
% \end{align}
% where $r(t, \zvec') = t\zvec', t\in[0,1]$ and $a=\epsilon/||\zvec'||$. $\epsilon$ is a hyper-parameter to determine how flatten $f_i(r(t, \xvec_c))$ is when $t\rightarrow 1$.
% \end{definition}


% In Robust Neighbor Search (SNS), we find a counterfactual example where the gradient of the model is almost zero. Intuitively, this gives a better approximation of finding a point far away from a deep model's decision boundary, as this suggests that for at least a small neighborhood around that point, there is little change in the model's decision. This gives intuition for why small perturbations in the model's decision boundary may be less likely to induce a change of prediction at that counterfactual point, making SNS counterfactuals less susceptible to invalidation across similar models. Notice that SNS counterfactuals have an invalidation rate of 1\% for the Seizure dataset over leave-one-out changes, and a 0\% invalidation rate for German Credit models over leave-one-out changes.

% Interestingly, these improvements in invalidation rate do not come at too high of a cost, at least in comparison to data-manifold based methods.

==> abstract.tex <==
% !TEX ROOT=./neurips_2021.tex

With deep learning models being used in more and more sensitive applications, the ability to explain their outputs in deployment is paramount. 
One explanation method commonly forwarded as a method of explaining high-stakes model decisions, is a \emph{counterfactual example}: for an input $x$ requiring an explanation, its counterfactual example is the nearest point $x'$ that produces a desired outcome from a model (e.g., the nearest potential accepted loan application to a rejected loan application).
Counterfactuals are often discussed under the assumption that the decision system on which they will be used is static. However, during real model deployments, there are often retrainings to ensure consistent optimal behavior. Thus, in order to be effective, explanation methods should be consistent in the presence of such small changes to a model. In this paper, we demonstrate that counterfactual examples are \emph{not} consistent similar deep models with \emph{arbitrary} differences in training environment, such as random seed or one-point difference in the training set. 
We demonstrate that increasing counterfactual cost (i.e. distance from the original input) to mitigate inconsistency, as suggested by some prior work, is not always a reliable method in deep models. 
%Additionally, common-sense  intuitions on how to fix this behavior, such as requiring counterfactual examples with high confidence, do not mitigate this behavior sufficiently well in deep models. 
Rather, we theoretically motivate how generating stable counterfactuals in deep models can be accomplished by locating points with \emph{low local Lipschitz constants in model's loss}. Motivated by this result, we provide a new counterfactual search method, robust neighbor search (RNS), that generates consistent counterfactuals across similar deep models by searching for counterfactual examples with low local Lipschitz constants.

%$\emily{As Zifan has noted throughout my introduction, I don't get to the meat of the paper until most of the way through this abstract. Is this ok? Thoughts on this?}


%NOTE ON ADVERSARIAL VS COUNTERFACTUALS:
% Theoretically, these are the same thing. The context is what determines the difference between these two ideas: adversarial examples are essentially a turing test for deep image networks, and counterfactual examples are an explanation method largely for tabular data. We plant ourselves solidly in the camp of counterfactruals. Firstly, we only consider work with tabular data, where the main condition of an adversarial example (that the differences between the original point and adversarial example are imperceptible) is not really well-defined---how can two different tabular points be imperceptibly different? And we do not meander into the main domain of adversarial examples, images, as what a "similar nearby image" is that can be used for explanation is currently being investigated by the research literature (cite few recent papers).
%
%and occaisionally a difference in desiderata adversarial examples require that the differences between input and adversarial example are imperceptible, which is not required in counterfactuals examples.
%  From the perspective of context, we plant ourselves solidly in the 
% 

%Idea: increase applicability of the paper by saying this is also about transferrable counterfactuals.

% \emph{Counterfactual examples}, are an explanation technique that has received much attention in the literature, and is forwarded as a method of explaining high-stakes model decisions, such as credit risk models. Since these explanations are ostensibly to be used during deployment, it is important that they 
% The 


% Thus, explanation methods should be consistent in the presence of small changes to a model, for example as a result of re-training while in deployment: i.e. once a counterfactual example is generated, it should produce the same desired result in a model even if that model is retrained.
% We demonstrate the extent of counterfactual invalidation, i.e. a counterfactual no longer producing the desired output, between similar deep models with \emph{arbitrary} differences in training environment, such as random seed or one-point difference in the training set. 
% We show that some common sense intuitions on how to lower invalidation rate do not hold sufficiently well in deep models to mitigate this problem: namely, generating higher confidence counterfactuals, and generating higher cost counterfactuals. 
% To mitigate this problem, we prove that models with a bounded Lipschitz constant will have lower counterfactual invalidation than unbounded models, and empirically verify our result. 
% Further, we provide a new counterfactual search method, robust neighbor search (RNS), that generates counterfactual with a low invalidation rate while maintaining a low cost.


==> background.tex <==
%!TEX root=paper.tex
\begin{itemize}
\item -Def of model duplicity
\item -def of CFs
\item -def of invalidation
\end{itemize}


==> emilyseval.tex <==
% !TEX ROOT=./neurips_2021.tex
\section{Evaluation}\label{sec:evaluation}
In this section, we evaluate the extent of invalidation across five different counterfactual generation methods, including Stable Neighbor Search, over models trained with two sources of randomness in setup: \emph{1)} initial weights, and \emph{2)} leave-one-out differences in training data.
Our results show that Stable Neighbor Search consistently generates counterfactuals with lower invalidation rates than all other methods, in many cases eliminating invalidation altogether on tested points. 
Additionally, despite not explicitly minimizing cost, SNS counterfactuals manage to maintain low cost relative to other methods that aim to minimize invalidation.

\subsection{Setup}
\paragraph{Data.} Our experiments encompass several tabular classification datasets from the UCI database~\cite{uci}, including: German Credit, Taiwanese Credit-Default, Seizure, and Cardiotocography (CTG). 
We also include FICO HELOC~\cite{fico} and Warfarin Dosing~\cite{international2009estimation}. 
All datasets have two classes except Warfarin, where we assume that the most favorable outcome (class 0) is the desired counterfactual for the other classes, and vice versa.
Further details of these datasets are included in Appendix~\ref{appendix:experiment-details-datasets}.

\paragraph{Baselines.} 
We compare SNS with the following baselines in terms of the invalidation rate. 
Further details about how we implement and configure these techniques are found in Appendix~\ref{appendix:experiment-detail-baselines}.
\begin{description}
\item[Min-Cost $\ell_1/\ell_2$~\cite{wachter2018counterfactual}:] We implement this by setting the appropriate parameters for the elastic-net loss~\cite{chen2018ead} in ART~\cite{art2018}.
\item[Min-$\epsilon$ PGD~\cite{madry2018towards}:] We perform Projected Gradient Descent (PGD) for an increasing sequence of $\epsilon$ until a counterfactual is found. 
\item[Carlini-Wagner (CW)~\cite{carlini2017towards}:] This method  was originally proposed to find high-confidence, low-cost adversarial examples, and often succeeds when PGD fails.
\item[Pawelczyk et al.~\cite{pmlr-v124-pawelczyk20a}:] This method attempts to find counterfactual examples \emph{on the data manifold}, that are therefore more resistent to invalidation, by searching the latent space of a variational autoencoder, rather than the input space.
\item[Looveren et al.~\cite{van2019interpretable}:] This method minimizes an elastic loss combined with a term that encourages finding examples on the data manifold.
\end{description}
We note that two of these baselines (PGD and CW) were originally proposed in the context of adversarial adversarial examples~\cite{szegedy2013intriguing}. 
As has been noted in prior work~\cite{freiesleben2020counterfactual,browne2020semantics,sokol2019counterfactual,wachter2018counterfactual}, the problem of finding adversarial examples is mathematically identical to that of finding counterfactual examples. 
While solution sparsity is sometimes noted as a differentiator between the two, we note that techniques from both areas of research can be used with various $\ell_p$ metrics.
We measure cost in terms of both $\ell_1$ and $\ell_2$ norms, providing $\ell_2$ in the main body and $\ell_1$ in Appendix~\ref{appendix:ell1-results}.
% As the difference between these adversarial and counterfactual examples is an area of active research, we do not endeavor to solve this question.


\begin{table}[t]
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
            \multicolumn{13}{c}{\emph{Invalidation Rate}} \\
            \toprule 
            \textbf{Method}&\multicolumn{2}{c}{German Credit} & \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{CTG} & \multicolumn{2}{c}{Warfarin}&\multicolumn{2}{c}{HELOC}& \multicolumn{2}{c}{Taiwanese Credit}\\
            \textbf&LOO & RS & LOO  & RS&LOO& RS&LOO & RS & LOO  & RS&LOO & RS \\
            \midrule
            Min. $\ell_1$ & 0.34 & 0.52 & - & - & 0.07 &  0.29& 0.44 & 0.35 & 0.30 &0.43 &0.30 & 0.78\\
            Min. $\ell_2$ &0.36 & 0.56 & 0.64 & 0.77 & 0.48 & 0.49& 0.35 &0.3 &0.55 & 0.61 & 0.27&0.72\\
            Looveren et al. & 0.25 & 0.40 & 0.48 & 0.54 & 0.11&0.18 & 0.26 & 0.25 & 0.25 & 0.34& 0.29& 0.53\\
            Min. $\epsilon$ PGD & 0.28 &  0.61 & 0.94 & 0.94& 0.02& 0.11 &0.10& 0.12& 0.04 & 0.11 &0.04 & 0.24\\
            $\quad \quad$+SNS & \textbf{0.00} & 0.13 &0.03 & 0.15 & \textbf{0.00} & \textbf{0.00} &0.01& 0.02& 0.00&  \textbf{0.00} &\textbf{0.00} & 0.11\\
            CW & 0.39 & 0.55 & 0.68&0.83& -&-& -&-& 0.01&0.05 &0.07&0.19\\
            $\quad \quad$+SNS & 0.01 & \textbf{0.05} & \textbf{0.02} & 0.13& - &-& -&-&0.00&\textbf{0.00}&\textbf{0.00}&\textbf{0.01}\\
            Pawelczyk et al. & 0.2 &0.35 &0.16 &\textbf{0.12} &0.00&0.06 &0.02&0.01& 0.04& 0.05& 0.01 &0.20\\
            % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
            % \rowcolor{black!5} \textsuperscript{16}O & 0 & 99.96 & -&& &\\
            % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
            \bottomrule
            \multicolumn{13}{c}{} \\
            \multicolumn{13}{c}{\emph{Counterfactual Cost ($\ell_2$)}} \\
            \toprule 
            \textbf{Method}&\multicolumn{2}{c}{German Credit} & \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{CTG} & \multicolumn{2}{c}{Warfarin}&\multicolumn{2}{c}{HELOC}& \multicolumn{2}{c}{Taiwanese Credit}\\
            \midrule
            Min. $\ell_1$ & \multicolumn{2}{c}{1.72} & \multicolumn{2}{c}{-}& \multicolumn{2}{c}{0.17}&\multicolumn{2}{c}{0.50}&\multicolumn{2}{c}{0.24}& \multicolumn{2}{c}{1.56}\\
            Min. $\ell_2$ & \multicolumn{2}{c}{4.49} & \multicolumn{2}{c}{8.23}& \multicolumn{2}{c}{0.06}&\multicolumn{2}{c}{0.54}&\multicolumn{2}{c}{0.11}& \multicolumn{2}{c}{2.65}\\
            Looveren et al. & \multicolumn{2}{c}{5.37} & \multicolumn{2}{c}{8.40}& \multicolumn{2}{c}{0.11}&\multicolumn{2}{c}{1.03}&\multicolumn{2}{c}{0.45}& \multicolumn{2}{c}{2.82}\\
            Min. $\epsilon$ PGD & \multicolumn{2}{c}{1.02} & \multicolumn{2}{c}{1.36}& \multicolumn{2}{c}{0.12}&\multicolumn{2}{c}{0.33}&\multicolumn{2}{c}{0.32}& \multicolumn{2}{c}{0.75}\\
            % CW &  &  & && &\\
            CW &  \multicolumn{2}{c}{0.37} & \multicolumn{2}{c}{2.52}& \multicolumn{2}{c}{-}&\multicolumn{2}{c}{-}&\multicolumn{2}{c}{0.19}& \multicolumn{2}{c}{0.77}\\
            \bottomrule
            % PGDs &  && && &\\
            PGD+SNS &\multicolumn{2}{c}{3.01} & \multicolumn{2}{c}{6.10}& \multicolumn{2}{c}{\textbf{0.22}}&\multicolumn{2}{c}{\textbf{0.50}}&\multicolumn{2}{c}{1.79}& \multicolumn{2}{c}{\textbf{2.78}}\\
            % CW &  &  & && &\\
            CW+SNS & \multicolumn{2}{c}{\textbf{2.63}} & \multicolumn{2}{c}{\textbf{6.01}}& \multicolumn{2}{c}{-}&\multicolumn{2}{c}{-}&\multicolumn{2}{c}{1.75}& \multicolumn{2}{c}{3.37} \\
            Pawelczyk et al. & \multicolumn{2}{c}{7.15} & \multicolumn{2}{c}{13.7}& \multicolumn{2}{c}{1.07}&\multicolumn{2}{c}{2.62}&\multicolumn{2}{c}{\textbf{1.35}}& \multicolumn{2}{c}{4.24}\\
            \midrule
            \textbf{$R^2$} & \multicolumn{2}{c}{0.048} & \multicolumn{2}{c}{0.025}& \multicolumn{2}{c}{0.00}&\multicolumn{2}{c}{0.007}&\multicolumn{2}{c}{0.14}& \multicolumn{2}{c}{0.00}\\%$HELOC: 3.8\cdot10^{-10}$}\\ CTG: 2.294e-7
            \bottomrule
            \\
        \end{tabular}%
        }
        \caption{The consistency of counterfactuals measured by invalidation rates. The average $\ell_2$ cost of different methods are also included. Results are aggregated over 100 networks for each experiment, i.e. calculating invalidation over differences in random seed and leave-one-out changes to the training set. Lower invalidation rates and cost are more desirable. For $\ell_2$ cost, the best results are highlighted among three methods (separated by a line) with lower invalidation rates. If a method has significantly low success rate in generating counterfactual examples, we report `-' in the table. In the last line of the table, we present the $R^2$ correlation coefficient from a linear regression predicting invalidation percentage from cost. Small values indicate weak correlation.}
        \label{table_IV}
        \end{table}

\paragraph{Implementation of SNS.} SNS begins with a given counterfactual example $\zvec$ as mentioned in Def.~\ref{def:SNS}, which are generated by Min. $\epsilon$ PGD or CW in our evaluations. The only hyper-parameter in SNS is $\alpha$ which is proportional to the radius of the local region where we want to minimize the local Lipschitz constant. We find the resulting invalidation rate for SNS is not very sensitive to the choice of $\alpha$. We use $\alpha=0.5$ in our all experiments and we include the sensitivity analysis in Appendix~\ref{appendix:experiment-detail-sensitivity-of-alpha}. 

\paragraph{Retraining Controls.}
We prepare different models for the same dataset using Tensorflow 2.3.0 and all computations are done using a Titan RTX accelerator on a machine with 64 gigabytes of memory. 
We control the random seeds used by both numpy and Tensorflow, and enable deterministic GPU operations in Tensorflow~\cite{tf-determinism}. 
We evaluate the invalidation rate of counterfactual examples under changes in retraining stemming from the following sources (see Appendix~\ref{appendix:experiment-detail-retraining} for more details on our training setup): 
\begin{description}
    
    \item[Leave-One-Out (LOO):] We select a random point (without replacement) to remove from the training data. Network parameters are initialized with the same values across runs.
    
    \item[Random Seed (RS):] Network parameters are initialized by incrementing the random seed across runs, while other hyperparameters and the data remain fixed.

\end{description}
We note that these sources of variation do not encompass the full set of sources that we are relevant to counterfactual invalidation, such as fine-tuning and changes in architecture or other hyperparameters.
However, they are straightforward to control, produce very similar models that nonetheless tend to invalidate counterfactuals, and they are not dependent on any deployment or data-specific considerations in the way that fine-tuning changes would be.
While we hope that our results are indicative of what might be observed across other sources, exploring invalidation in more depth in particular applications is important future work.

\paragraph{Metrics.} We benchmark the consistency of counterfactuals generated by different algorithms, we compute the mean invalidation rate (Def.~\ref{def:invalidation-rate}) over the validation split of each dataset.
To calculate the extent of correlation between cost and invalidation, as discussed in Section~\ref{sec:invalidation}, we perform a linear regression (\texttt{scipy.linregress}) between the costs for each valid counterfactual, across all five methods, with its invalidation rate across both LOO and RS differences. 
Table~\ref{table_IV} reports the resulting $R^2$ for each dataset.

\paragraph{Methodology.}
For each dataset, we train a ``base'' model and compute counterfactual examples using the five methods for each point in the validation split.
For each set of experiments (LOO or RS), we train $100$ additional models, and compute the invalidation rate between the base model and the $100$ variants. 
The results are shown in Table~\ref{table_IV}.

% For experiments investigating invalidation between models with a one-point difference in training set, we also set the numpy random seed, and use the same random initialization of model parameters across models. 
% For experiments evaluating invalidation over different random initialization, we set a new random seed for each model that is trained, and keep the same training set. 


%The German Credit, Seizure, and CTG models models have
% three hidden layers, of size 128, 64, and 16.  German Credit,
% Seizure, All models are trained for 100 epochs. German Credit models are trained
% with a batch size of 32,  Seizure ...
% The Lipschitz models are trained with the deel-lip package~\cite{} to ensure a specified Lipschitz constant throughout the entire model. They have the same architecture, batch size, training sets, and random seeds as the non-Lipschitz models. We train models with to have Lipschitz constant of 1, except when this deteriorates performance drastically, in which case we use a Lipschitz constant of 3 (CTG dataset).





\subsection{Results}
    
% \begin{table}[t]
%     % \begin{tabular}{l|llll|llll}
%     % \toprule
%     %         & \multicolumn{8}{c}{Average Invalidation Rate, Counterfactual Cost} \\
%     %         & \multicolumn{4}{c|}{Random Seed} & \multicolumn{4}{c}{Leave-one-out} \\
%     % Dataset & PGD & CW & AE & SNS & Min Cost & High Confidence & Data Manifold &  SNS \\
%     % \midrule
%     %  German Credit &  &  &  & & & & & \\
%     %  Seizure &  &  &  & & & & &  \\
%     %  Adult &  &  &  &  & & & & \\
%     %  Warfarin &  &  &  &  & & & &  \\
%     %  HELOC &  &  &  &  & & & &  \\
%     %  Taiwanese Credit &  &  &  & & & & &  \\
%     % \bottomrule
%     % \end{tabular}
%     \begin{tabular}{ccccccc}
%         \multicolumn{7}{c}{Invalidation Rate  (Leave-One-Out)} \\
%         \toprule 
%         \textbf{Method}&German Credit & Seizure & CTG  & Warfarin&HELOC& Taiwanese Credit\\
%         \midrule
%         Wachter et al. &  &  &  & & & \\
%         Min. $\epsilon$ PGD & 0.28 & 0.94 & 0.02&0.10&0.04 &0.04\\
%         PGD+SNS & \textbf{0.00} &0.03 &\textbf{0.00} &0.01&0.00& \textbf{0.00}\\
%         CW & 0.39 & 0.68& -&-& 0.01&0.07\\
%         CW+SNS & 0.01 & \textbf{0.02} & - &-&0.00&\textbf{0.00}\\
%         Pawelczyk et al. & 0.2 &0.16 &0.0&0.02& 0.04&0.01\\
%         Looveren et al. & 0.25 & 0.48 &  & & & \\

%         % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
%         % \textsuperscript{16}O & 0 & 99.96 & -&& &\\
%         % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
%         \bottomrule
%         \\
%         \multicolumn{7}{c}{Invalidation Rate (Random Seed)} \\
%         \toprule 
%         \textbf{Method}&German Credit & Seizure & CTG  & Warfarin&HELOC& Taiwanese Credit\\
%         \midrule
%         Wachter et al. &  &  &  & & & \\
%         Min. $\epsilon$ PGD & 0.61 & 0.94 &0.11 &0.12& 0.11&0.24\\
%         PGD+SNS & 0.13 & 0.15& \textbf{0.00}&0.02&\textbf{0.00}& 0.11\\
%         CW & 0.55 &0.83  & -&-&0.05 &0.19\\
%         CW+SNS & \textbf{0.05} &  0.13& -&-&\textbf{0.00}&\textbf{0.01}\\
%         Pawelczyk et al. & 0.35 & \textbf{0.12}&0.06 &0.01&0.05 &0.20\\
%         Looveren et al. &0.40  & 0.54 &  & & & \\
%         % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
%         % \textsuperscript{16}O & 0 & 99.96 & -&& &\\
%         % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
%         \bottomrule
%         \\
%         \multicolumn{7}{c}{$\ell_2$ Cost of Counterfactual Explanations} \\
%         \toprule 
%         \textbf{Method}&German Credit & Seizure & CTG & Warfarin&HELOC& Taiwanese Credit\\
%         \midrule
%         Min. $\epsilon$ PGD & 1.02 & 1.36& 0.12&0.33&0.32& 0.75\\
%         % CW &  &  & && &\\
%         CW &  0.37 &  2.52&  -&- & 0.19&0.77\\
%         \bottomrule
%         % PGDs &  && && &\\
%         PGD+SNS &3.01 &6.10 &0.22 &0.50&1.79&\textbf{2.78} \\
%         % CW &  &  & && &\\
%         CW+SNS & \textbf{2.63} & \textbf{6.01} & - & - &1.75&3.37\\
%         Pawelczyk et al. &7.15  &13.7 &1.07&2.62& \textbf{1.35}&4.24\\
%         Looveren et al. & 5.37 & 8.40 &  & & & \\

%         % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
%         % \textsuperscript{16}O & 0 & 99.96 & -&& &\\
%         % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
%         \bottomrule
%         \\
%     \end{tabular}
%     \caption{The consistency of counterfactuals measured by invalidation rates. The average $\ell_2$ cost of different method are also included. Results are aggregated over 100 networks, respectively. Lower invalidation rate and lower cost are better. For $\ell_2$ cost, the best results are highlights among four methods (separated by a line) with relatively lower invalidation rates. CW has significantly lower success rate in finding counterfactuals for CTG and Warafin and is therefore not reported in the table.}
%     \label{table_IV}
%     \end{table}


% \paragraph{Invalidation, Cost, Success Rate Calculations.}
% To calculate invalidation, we generate a counterfactual in baseline model $h_S$ for each point in the test set for all methods evaluated. Success rate represents how many counterfactuals generated in fact are of the desired class, which we check by verifying the predictions of the counterfactuals generated in the baseline model. We calculate counterfactual cost by calculating the $\ell_2$ norm of the difference of the origin point and the counterfactual for each point in the test set, and averaging over the test set.
% To calculate invalidation rate, we first calculate the predictions of these counterfactuals in the $100$ nearby models with either a different random seed or a one-point difference in the training set (separately). We calculate the percentage of the time each counterfactual is invalidated, i.e. retuSns a different outcome in a nearby model, over these 100 models. Then we take the average of this percentage over the entire test set to get the invalidation percentage reported in Table~\ref{table_IV}.  

% \begin{table}[t]
%         \begin{tabular}{ccccccc}
%             \multicolumn{7}{c}{$\ell_2$ Cost of Consistent Counterfactual Explanations} \\
%             \toprule 
%             \textbf{Approach}&German Credit & Seizure & Adult  & Warfarin&HELOC& Taiwanese Credit\\
%             \midrule
%             % PGDs &  && && &\\
%             PGD+SNS &3.01 &6.10 &1.47 &0.50&1.79&\textbf{2.78} \\
%             % CW &  &  & && &\\
%             CW+SNS & \textbf{2.63} & \textbf{6.01} &\textbf{1.43}  &&1.75&3.37\\
%             AE &7.15  &13.7 &1.97&2.62& \textbf{1.35}&4.24\\
%             % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
%             % \textsuperscript{16}O & 0 & 99.96 & -&& &\\
%             % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
%             \bottomrule
%             \\
%             % \multicolumn{7}{c}{$\ell_2$ Cost (Random Seed)} \\
%             % \toprule 
%             % \textbf{Approach}&German Credit & Seizure & Adult  & Warfarin&HELOC& Taiwanese Credit\\
%             % \midrule
%             % PGDs & 1.9 & 1.30 &1.00 && &\\
%             % $\quad \quad$+SNS & 2.7 &5.24 & &&& \\
%             % CW &  & 1.49 & && &\\
%             % $\quad \quad$+SNS &  &  & &&&\\
%             % AE &  & 13.7 & && &\\
%             % % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
%             % % \textsuperscript{16}O & 0 & 99.96 & -&& &\\
%             % % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
%             % \bottomrule
%             % \\
%         \end{tabular}
%         \caption{$\ell_2$ Cost of Counterfactual ... TODO}
% \end{table}

Looking at the invalidation results in Table~\ref{table_IV}, the most salient trend is apparent in the low invalidation rates of SNS compared to the other methods.
SNS achieves the lowest invalidation rate across all datasets in both LOO and RS experiments, except for on the Seizure dataset with RS variations, where there is a one-point difference in the invalidation rate. 
SNS generates counterfactuals with \emph{no} invalidation over LOO differences on German Credit, CTG, Heloc, and Taiwanese Credit. 
Notably, this is down from invalidation rates as high as 61\% from other methods on German Credit, and $\approx10-50\%$ on others.
On Seizure, which had IV rates as high as 94\% from other methods, SNS achieves just 2\% (LOO) and 13\% (RS) invalidation.
The closest competitor is the method of Pawelczyk et al.~\cite{pmlr-v124-pawelczyk20a}, which achieves zero invalidation in one case (CTG under LOO), but at significantly greater cost--in every case SNS produced less-costly counterfactuals, and in nearly every case the margin between the two is greater than $2\times$.

As discussed in Section~\ref{sec:invalidation}, while increasing cost is not a reliable way to generate stable counterfactuals for deep models, our results do show that stable counterfactuals tend to be more costly. 
The data suggests that greater-than-minimal cost appears to be necessary for stability. 
While SNS counterfactuals are much less costly than those generated by Pawelczyk et. al, they are consistently more costly than other methods that aim minimize cost without other constraints. 
Notably, Table~\ref{table_IV} shows that the correlation between cost and invalidation is quite weak: the \emph{maximum} $R^2$ over all datasets is $0.05$ (German Credit), while most of the other datasets report coefficients that are orders of magnitude smaller.


% \subsection{Cost-Invalidation Trade-off}

% \paragraph{Calculating Correlation between Cost and Invalidation.}
% We calculate the correlation between counterfactual cost and invalidation for each dataset by pooling the results of all counterfactual example methods together for each dataset, and using scipy.stats.lingress to calculate the least-squares regression between counterfactual cost and average invalidation rate over the $100$ models with either a leave-one-out difference in the training set, or trained with a different random seed, described earlier. We report the correlation through the r-value that the function retuSns directly.  


%We note that our results connecting instability to model loss point to an interesting intuition as to why counterfactuals from the data support are more stable: boundary changes \emph{outside} of the data distribution are much more unpredictable than boundary changes \emph{inside} the data distribution, as these changes do not affect the model's loss during training. Thus, data support counterfactuals may be more stable simply by virtue of the model's decision surface being more stable in areas around points in the data distribution, a phenomenon also noted by --et al~\cite{googlepaper}. 
%We note that SNS does not currently consider the feasibility of the counterfactuals it generates, nor does it consider whether the counterfactuals generated produce a realistic point. This may be made possible by limiting the search space of SNS, but we leave incorporating these desiderata as future work.

==> eval.tex <==
% !TEX ROOT=./neurips_2021.tex

%We demonstrate the high level of counterfactual invalidation between deep models with arbitrary changes that do not affect the learning rule--namely, one-point differences in the training set, and changes in random initialization. We show that minimum-cost methods of generating counterfactuals in deep models are invalidated between 10\%-96\% of the time. Further, 
After noting the high invalidation rate of counterfactual explanations in deep models---with counterfactuals returning inconsistent predictions between nearby models up to 96\% of the time---we demonstrate that increasing counterfactual cost, a mitigation technique suggested by prior work, is not a reliable method to generate stable counterfactuals in deep models.
%the cost-invalidation tradeoff posited by other works is not a sufficient condition for choosing stable counterfactuals in deep models--that is, it is possible to get higher-cost counterfactuals with higher invalidation rates than lower-cost alternatives. This points to the fact that a higher-than-minimal counterfactual cost is necessary for a counterfactual to be stable, (i.e. points that are the \emph{closest point} of the opposite class will always lie on the decision boundary and are likely to be invalidated), but high cost is not a sufficient condition to ensure stability. And, there is no well-motivated way to choose between counterfactuals of different costs to ensure stability. 
%For changes so minuscule, counterfactuals should be nearly completely consistent between models--i.e. that is, a counterfactual generated in one model should produce the same prediction in the same model trained with a different random seed, or small change to the training set. 
% \subsection{Minimum-cost Counterfactual Invalidation in Deep Models.} 
% Pawelczyk et al. have demonstrated the problem of counterfactual invalidation in linear and random forest models, especially for minimum-cost counterfactuals. We show that this problem persists in deep models as well. We see in Table ~\ref{} that minimum cost counterfactuals change their prediction between models as often as 96\% of the time.
\subsection{Counterfactual Cost and Invalidation in Deep Models}
As we demonstrate in more detail in Section ~\ref{sec:evaluation}, counterfactual invalidation is a problem in deep networks on real data: countefactuals produce inconsistent outcomes in duplicitous models up to 96\% of the time. 
%Pawelczyk et al.~\cite{pmlr-v124-pawelczyk20a} have drawn attention to the problem of counterfactual invalidation in duplicitous linear and random random forest models. %As we demonstrate in Section ~\ref{sec:evaluation}, this problem also holds in duplicitous \emph{deep} models, with invalidation rates as high as 96\%. 
Previous work investigating the problem of counterfactual invalidation, in duplicitious linear and random forest models~\cite{pmlr-v124-pawelczyk20a}, and due to larger distributional shifts~\cite{rawal2021i}, have pointed to increasing counterfactual cost as a potential mitigation strategy.
%Previous work has pointed out the relationship between counterfactual cost and invalidation rate, 
They prove that higher cost counterfactuals will lead to lower invalidation rates in linear models in expectation~\cite{rawal2021i}, and demonstrate their relationship in a broader class of well-calibrated models~\cite{pmlr-v124-pawelczyk20a}. 

While an interesting challenge to the perspective that low cost counterfactuals should be preferred, we show that insight is insufficient to determine which counterfactual has a greater chance of being stable at generation time in deep models. %While it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary, there is no consistent inverse relationship between counterfactual cost and invalidation, so it is not a reliable metric to use when generating counterfactuals to \emph{ensure} stability across nearby models, especially for deep models.
% \begin{observation}\label{observation:cost_insufficient_signal}
% Even in linear models, high cost counterfactuals do not guarantee a low invalidation rate.
% \end{observation}
The intuition that a larger distance between input and counterfactual will lead to lower invalidation rests on the assumption that the distance between $x$ and $x_c$ is indicative of the distance from $x_c$ from the decision boundary, with a higher distance making $x_c$'s prediction more stable under small perturbations to that boundary. This holds well in a linear model, where there is only one boundary~\cite{rawal2021i}. However, in deep models, this intuition can break down. The complex decision surfaces of deep networks mean that going farther away from a point across the \emph{nearest} boundary may in fact lead to being closer to an \emph{different} boundary, as we show in Lemma~\ref{lemma:deep_boundaries}.
%However counterfactual cost, $|x-x_c|_p$, i.e. the distance from the input point requiring an explanation, does not correspond exactly to the distance between a counterfactual the decision boundary. We show this in Figure ~\ref{fig:toy-linear}, created by training two different linear models (differing only by random seed) on a synthetic dataset of half-moons, pictured alongside in Figure ~\ref{fig:toy-data}. The black and grey areas are where the two models predict the blue class. See that point for $x_4$ and its corresponding counterfactual, the counterfactual cost is relatively large due to the fact that $x_c$ is further away from $x$ in a direction parallel to the boundary.
%Thus, while cost and invalidation may share an inverse relationship in expectation, cost alone is an insufficient signal to follow when searching for consistent counterfactuals.
%are certainly related--- for example, it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is an insufficient signal to follow when searching for consistent counterfactuals.
\begin{Lemma}\label{lemma:deep_boundaries}\todo{turn this into a better lemma. Do we want to say something directly about IV, or is just the boundaries enough?}
%Consider a deep model $F(\theta, \xvec)$ with 
In deep models, a higher distance from the \emph{closest} boundary does not guarantee being far away from \emph{any} boundary.
\end{Lemma}
\begin{proof}
We prove this lemma by demonstration. Consider Figure ~\ref{fig:toy-non-linear}, which we created by training a DNN on the synthetic dataset pictured in Figure ~\ref{fig:toy-dataset}. The grey shaded regions denote where the model predicts the blue class. See that for point $x_1$, the higher-cost counterfactual generated for that point in the is actually closer to a decision boundary than the lower-cost counterfactual.
\end{proof}
Thus, cost is not a reliable metric to determine counterfactual stability at generation time: a counterfactual example with a higher cost, while perhaps further from the nearest boundary to the origin point, may in fact be closer to some boundary $b'$, making its prediction potentially equally or even more sensitive to small perturbations to the decision surface.

We can see this demonstrated in Figure ~\ref{fig:toy-non-linear}, which compares the decision surfaces of two DNNs trained on the same synthetic dataset pictured. The grey shaded regions denote where one model predicts the blue class, the darker grey shaded regions show where the other model predicts the blue class, and the black areas are where the decision surfaces overlap. Note that the higher cost counterfactual for point $x_1$ generated in the light grey model is invalidated in the dark grey model, as it is closer to a decision boundary. %Even further, even counterfactuals equally far from a decision boundary may have different invalidation behavior, as demonstrated by point $x_2$. We give a principled explanation of why this may be the case in Section ~\ref{sec:method}. \todo{Maybe we shouldn't have this point? I thought our intuition was that we are searching for a point where the model's decision surface is stable/smooth...and I thought saying the loss was stable/smooth was tantamount to the model being stable/smooth. Is this not true?} 

We demonstrate that there is no strong correlation between cost and invalidation percentage in deep models on real datasets in Section ~\ref{sec:evaluation}, by showing that counterfactuals with higher costs may have higher invalidation rates than counterfactuals with lower cost~\ref{table:results}, and that the $R^2$ coefficient between counterfactual cost and invalidation is \emily{TODO:fill in.}
%it highly likely to be invalidated
%even if one counterfactual is further from the boundary which it had to cross to change prediction from its origin point---i.e. its nearest boundary--this does not guarantee that it is far away from \emph{any} decision boundary. Following the intuition that distance 
Thus, while cost and invalidation are certainly related--- for example, it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is not enough to determine which, out of a series potential counterfactuals, may be the most consistent. In the next section, we demonstrate how, perhaps counterintuitively, requiring that counterfactuals be \emph{confidently predicted} is also ineffective at ensuring consistency. Following this, we motivate how a \emph{low local Lipschitz constraint} of a point in a region of a model serves as a reliable signal to find stable counterfactuals in deep models.

%Thus, while cost and invalidation are certainly related--- for example, it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is not enough to determine which, out of a series potential counterfactuals, may be the most consistent. In the next section, we demonstrate how, perhaps counterintuitively, requiring that counterfactuals be \emph{confidently predicted} is also ineffective at ensuring consistency. Following this, we motivate how a low local Lipschitz constant of a point \emph{on the generating model's loss} serves as a reliable signal to find stable counterfactuals in deep models.

%Thus, naively maximizing cost may not be a reliable, or optimal, method to generate stable counterfactuals. However, in a broader sense, the intuition that counterfactuals farther away from a model's decision boundary will lead to lower invalidation is helpful, and gives us a direction of inquiry to find a metric we can use to determine the reliability to a counterfactual: in order to update this intuition to deep models, we must search for a point that is far away from \emph{any} decision boundary. We build upon this intuition in Section ~\ref{sec:method}. 

%Instead, to generate counterfactuals with stable predictions across similar models,  we must follow some other signal which correlates more strongly with invalidation behavior.
%Instead, to generate counterfactuals with stable predictions across similar models, To do this, we need to find another signal to follow which corresponds more closely w
%in order to find counterfactual examples that are stable in their outcomes across models close to their generating model, we need to find a more reliable signal to foll
%In a broader sense, the intuition that counterfactuals farther away from a model's decision boundary will lead to lower invalidation is helpful, and gives us a direction of inquiry to find a metric we can use to determine the reliability to a counterfactual: in order to update this intuition to deep models, we must search for a point that is far away from \emph{any} decision boundary. 

%the point can be more costly in that it is further from the original point in a direction orthogonal to the boundary. So while it may be generally true that counterfactual with higher cost may be more consistent across nearby models than one of lower cost, it is unclear how to use cost as metric to choose between counterfactuals in order to increase consistency. We note that in gradient-based counterfactual methods, the generation of a higher-cost counterfactual in a direction parallel to the boundary is highly unlikely, but in data-support methods~\cite{}, especially hose using VAEs, this may well happen, as the counterfactual search is in a latent space, which may translate to the input space in unexpected ways. %It is worth pointing out that this may

%In deep models, even the intuition that a counterfactual example farther away from the decision boundary between $x$ and $x_c$ will mitigate invalidation will not always hold. The complex decision surfaces of deep networks mean that going farther away from a point across the \emph{nearest} boundary may in fact lead to being closer to a different boundary, as we demonstrate in Figure ~\ref{fig:toy-non-linear}, which we created by training two different DNNs, again differing only by random seed), the same synthetic dataset. See that for point $x_2$, two counterfactuals with the same cost have different invalidation rates. And, for point $x_1$, the lower-cost counterfactual pictured for that point is actually more stable, as it is further from any boundary, than the higher-cost point. 

%We confirm these observations with demonstrations in Section ~\ref{sec:evaluation} that counterfactual examples generated in real models with common explanation methods can have similar costs but differing invalidation rates, or similar invalidation rates with differing costs. Thus, while cost and invalidation are certainly related--- for example, it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is not enough to determine which, out of a series potential counterfactuals, may be the most consistent. 
%a large distance from a model's decision boundary will prevent that point from changing prediction in a nearby model has more complications. In a deep model with a highly complex network of boundaries, going farther away from a point across the \emph{nearest} boundary may in fact lead to being closer to a different boundary. This fact also further complicates the use as counterfactual cost as a proxy for distance from the model's decision boundary, as counterfactuals farther away from the initial point may be closer to some model boundary. 
%We demonstrate this geometric intuition in Figure ~\ref{}, created by training two different DNNs (differing only by random seed) on a synthetic dataset of half-moons. The black and grey areas are where the two the decision boundaries of two models lies. See that for point $x_1$, the lower-cost counterfactual pictured for that point is actually likely to be more stable, as it is further from any boundary. 
% Previous work has demonstrated that counterfactuals in the support of the data distribution are more consistent across nearby models, but associated this gain with counterfactual cost~\cite{pmlr-v124-pawelczyk20a}. We display again in Figure ~\ref{} another intuition for why counterfactuals in the data support may decrease invalidation: as we see in the lower left of the figure boundary changes \emph{outside} of the data distribution are much more unpredictable than boundary changes \emph{inside} the data distribution, as these changes do not affect the model's loss during training. Thus, choosing such a counterfactual gives a higher chance that the model will not experience large perturbations in the area that may flip the prediction of the counterfactual.  In Section ~\ref{}, we will expand on this connection between a model's loss and invalidation rate to motivate our method of finding counterfactuals, \emph{Robust Neighbor Search}, to find counterfactuals with a low invalidation rate.
% However, data-based counterfactuals do not always lead to low invalidation, as even Pawelczyk et al. demonstrate--- and this still leaves the problem of finding a reliable method of finding consistent counterfactuals, since cost is not a reliable signal. In the next section, we consider \emph{confidence of prediction} of a counterfactual as a metric to approximate distance from the boundary in a deep network, and therefore, greater consistency.

\emily{Is this even worth saying? I'm tempted to take this out.}
\subsection{High Confidence Counterfactuals}

%In a broader sense, the intuition that counterfactuals farther away from a model's decision boundary will lead to lower invalidation is helpful, and gives us a direction of inquiry to find a metric we can use to determine the reliability to a counterfactual: in order to update this intuition to deep models, we must search for a point that is far away from \emph{any} decision boundary. 
One intuitive way to achieve this is to require that counterfactuals have a higher confidence in the generating model. However, as we show in the next section, this is largely ineffective in unconstrained deep models.

In order to better approximate achieving counterfactuals with higher distance from a decision boundary in deep models, it may seem natural to require counterfactuals to be confidently predicted. That is, we modify the definition of our counterfactual to be $x_c= \text{argmin}_{x_c | F(x_c)=c, f(x_c)>t} |x-x_c|_p$, where $t$ is a confidence threshold. Intuitively, a higher confidence threshold should point to a region that is far away from a decision boundary, as is the case in linear models.

However, as has been demonstrated by prior works in other contexts~\cite{}, high confidence does not necessarily coincide with a large distance to the boundary. In unconstrained, regularly trained deep networks, confidence is very badly callibrated. Thus, as we confirm in our results in Figure ~\ref{}, this requirement does not greatly reduce invalidation percentage. 
%old with linear observations in 
% We demonstrate the high level of counterfactual invalidation between deep models with arbitrary changes that do not affect the learning rule--namely, one-point differences in the training set, and changes in random initialization. We show that minimum-cost methods of generating counterfactuals in deep models are invalidated between 10\%-96\% of the time. Further, we demonstrate that the cost-invalidation tradeoff posited by other works is not a sufficient condition for choosing stable counterfactuals in deep models--that is, it is possible to get higher-cost counterfactuals with higher invalidation rates than lower-cost alternatives. This points to the fact that a higher-than-minimal counterfactual cost is necessary for a counterfactual to be stable, (i.e. points that are the \emph{closest point} of the opposite class will always lie on the decision boundary and are likely to be invalidated), but high cost is not a sufficient condition to ensure stability. And, there is no well-motivated way to choose between counterfactuals of different costs to ensure stability. 
% \subsection{Minimum-cost Counterfactual Invalidation in Deep Models.} 
% Pawelczyk et al. have demonstrated the problem of counterfactual invalidation in linear and random forest models, especially for minimum-cost counterfactuals. We show that this problem persists in deep models as well. We see in Table ~\ref{} that minimum cost counterfactuals change their prediction between models as often as 96\% of the time.
% \subsection{Counterfactual Cost and Invalidation in Deep Models}
% Previous work has pointed out the relationship between counterfactual cost and invalidation rate, proving that higher cost counterfactuals will lead to lower invalidation rates in linear models in expectation, and demonstrating their correlation in a broader class of well-calibrated models~\cite{rawal2021i,pmlr-v124-pawelczyk20a}.
% While an interesting challenge to the perspective that low cost counterfactuals should always be preferred, this insight is insufficient to determine which counterfactual has a greater chance of being stable at generation time. 
% \begin{observation}\label{observation:cost_insufficient_signal}
% Even in linear models, high cost counterfactuals do not guarantee a low invalidation rate.
% \end{observation}
% In linear models, the intuition that a larger distance between input and counterfactual will lead to lower invalidation rests on the assumption that this distance between $x$ and $x_c$ is indicative of the distance from $x_c$ from the decision boundary-- in a linear model, the further away a point is from the decision boundary, the less likely a small perturbation to the boundary will be to change that point's prediction~\cite{rawal2021i}. 
% However counterfactual cost, $|x-x_c|_p$, i.e. the distance from the input point requiring an explanation, does not correspond exactly to the distance between a counterfactual the decision boundary. We show this in Figure ~\ref{fig:toy-linear}, created by training two different linear models (differing only by random seed) on a synthetic dataset of half-moons, pictured alongside in Figure ~\ref{fig:toy-data}. The black and grey areas are where the two models predict the blue class. See that point for $x_4$ and its corresponding counterfactual, the counterfactual cost is relatively large due to the fact that $x_c$ is further away from $x$ in a direction parallel to the boundary.
% Thus, while cost and invalidation may share an inverse relationship in expectation, cost alone is an insufficient signal to follow when searching for consistent counterfactuals.
% \begin{observation}\label{observation:cost_insufficient_signal}
% In deep models, a higher distance from the \emph{closest} boundary does not guarantee being far away from \emph{any} boundary.
% \end{observation}
% In deep models, even the intuition that a counterfactual example farther away from the decision boundary between $x$ and $x_c$ will mitigate invalidation will not always hold. The complex decision surfaces of deep networks mean that going farther away from a point across the \emph{nearest} boundary may in fact lead to being closer to a different boundary, as we demonstrate in Figure ~\ref{fig:toy-non-linear}, which we created by training two different DNNs, again differing only by random seed), the same synthetic dataset. See that for point $x_2$, two counterfactuals with the same cost have different invalidation rates. And, for point $x_1$, the lower-cost counterfactual pictured for that point is actually more stable, as it is further from any boundary, than the higher-cost point. 
% We confirm these observations with demonstrations in Section ~\ref{sec:evaluation} that counterfactual examples generated in real models with common explanation methods can have similar costs but differing invalidation rates, or similar invalidation rates with differing costs. Thus, while cost and invalidation are certainly related--- for example, it is necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is not enough to determine which, out of a series potential counterfactuals, may be the most consistent. In the next section, we motivate how a \emph{low local Lipschitz constraint} of a point in a region of a model serves as a reliable signal to find stable counterfactuals in deep models.


%------potentially still useful---
%However, this still leaves the problem of finding a reliable method to find consistent counterfactuals--we have seen correlations an heuristics, but no well motivated method of choosing between counterfactuals with stability in mind.
%behind the idea that counterfactual cost correlates with to lower instability, i.e. using c
%Previous work has drawn a connection between the cost of a counterfactual, i.e. its distance from its original point, and invalidation chance in linear models~\cite{rawal2021i}. Intuitively, this makes sense, as in a linear model, if a counterfactual is far away from its generating point, it is more likely to be far away from the boundary as well--and (small) perturbations of the model's decision boundary are thus less likely to affect it. However, this geometric intuition breaks down in a deep model, where moving further away from one boundary can lead you to another. 

%While we can see from the results that there are certainly situations where increasing counterfactual cost can decrease invalidation (e.g. Adult, Wafarin), it is not guaranteed in a deep model (notice the relative consistency in invalidation percentage on the Seizure dataset, and that the German Credit Dataset retains high IV over high cost counterfactuals). Intuitively, increasing counterfactual cost is more likely to improve invalidation behavior in deep models which learn essentially linear functions, i.e. do not take advantage of the complexity of their hypothesis class. In this case, the model's decision surface may not be a hyper-complex network, but rather consist of only a few boundaries, in which case geometric intuitions from linear models will likely carry over.
%---
%$However, while simply increasing cost may be a poor method of achieving distance from a decision boundary in a deep model, this does not discount the idea that more stable counterfactuals can be found in regions far away from \textit{any} decision boundary in a deep model. However, as we empirically show further in Section ~\ref{RNS}, distance to the original point and distance from decision boundaries does not always correlate.
%OLD
% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|llll|llll}
% \toprule
%         & \multicolumn{8}{c}{Average Invalidation Rate} \\
% Dataset & German Credit & Seizure & Adult & Warafin & Taiwanese Credit & CTG &  Thyroid & ? \\
% \midrule
% Random Seed &  &  &  & & & & & \\
% LOO &  &  &  & & & & &  \\
% \bottomrule
% \end{tabular}}
% \end{table}
% \caption{Left: Graphs of invalidation (y-axis) percentage versus cost and confidence (both shown on the x-axis) for Seizure, German Credit, Adult and TBD datasets. Right: Difference between deep and linear train accuracies on these datasets, an indicator whether the complexity of a deep model was utilized in creating the decision function. (Similar train accuracies suggests the deep model did not take advantage of the complexity of its hypothesis class, leading to decision boundaries that may look more like a linear model's.) Notice that models with higher difference between deep and linear accuracies have a much higher invalidation rate, and this rate remains more stable over increasing counterfactual cost.}
%-------------------------------------------
% \subsection{Data Manifold Counterfactuals}

% While counterfactuals generated from the data distribution do often give \emph{lower} invalidation rates than low-cost methods, they are often only low in comparison to astronomical invalidation rates in other methods--e.g. 15\% as opposed to 96\%. However, a one in ten or even twenty chance of having a counterfactual invalidated for e.g. a loan application algorithm is still high, especially given that the counterfactuals generated by these methods are of much higher cost (~5x) than other methods of generating counterfactuals, so the effort put in to achieving these counterfactuals is much greater.
%-------------------------------------
%--old
%show that intuitions from prior work suggesting that higher-cost, or equivalently, high-confidence, counterfactuals are less likely to be invalidated do not always hold in deep models.
%, and higher-confidence counterfactuals are less likely to be invalidated, do not always hold, and requiring these things does not achieve sufficient stability across models.

% \begin{table}[]
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|lll|lll}
% \toprule
%         & \multicolumn{6}{c}{Average Invalidation Rate, Counterfactual Cost} \\
%         & \multicolumn{3}{c|}{Random Seed} & \multicolumn{3}{c}{Leave-one-out} \\
% Dataset & Min Cost & Higher Cost, Low IV & Higher Cost, High IV & Min Cost & Higher Cost, Low IV & Higher Cost, High IV \\
% \midrule
%  German Credit &  &  &  & & & & & \\
%  Seizure &  &  &  & & & & &  \\
%  Adult &  &  &  &  & & & & \\
%  Warfarin &  &  &  &  & & & &  \\
%  CTG &  &  &  &  & & & &  \\
%  Taiwanese Credit &  &  &  & & & & &  \\
% \bottomrule
% \end{tabular}}
% \end{table}
% \caption{Invalidation rates for minimum cost counterfactuals on }
%\subsection{Minimum-Cost Counterfactuals}
% Previous work has drawn a connection between the cost of a counterfactual, i.e. its distance from its original point, and invalidation chance in linear models~\cite{rawal2021i}. Intuitively, this makes sense, as in a linear model, if a counterfactual is far away from its generating point, it is more likely to be far away from the boundary as well--and (small) perturbations of the model's decision boundary are thus less likely to affect it. However, this geometric intuition breaks down in a deep model, where moving further away from one boundary can lead you to another. 
% While we can see from the results that there are certainly situations where increasing counterfactual cost can decrease invalidation (e.g. Adult, Wafarin), it is not guaranteed in a deep model (notice the relative consistency in invalidation percentage on the Seizure dataset, and that the German Credit Dataset retains high IV over high cost counterfactuals). Intuitively, increasing counterfactual cost is more likely to improve invalidation behavior in deep models which learn essentially linear functions, i.e. do not take advantage of the complexity of their hypothesis class. In this case, the model's decision surface may not be a hyper-complex network, but rather consist of only a few boundaries, in which case geometric intuitions from linear models will likely carry over.


==> idk.tex <==
% !TEX root = paper.tex

%\documentclass{standalone}

% \usepackage{pgfplots}
% \pgfplotsset{compat=1.16}
% \usepgfplotslibrary{groupplots}
% \usetikzlibrary{patterns}

% \begin{document}
\begin{tikzpicture}
\begin{groupplot}[%
	group style = {group size=6 by 1, horizontal sep=15pt, vertical sep=20pt}, 
	% classes={
	% 	a={mark=triangle*,blue},
	% 	b={mark=triangle*,green},
	% 	c={mark=triangle*,red},
	% 	d={mark=triangle*, black}
	% },
	footnotesize,
	% xlabel={Dimensions},
	% ylabel={Variance},
	xtick={1, 5, 10, 15, 20},
	%ytick={0, 5, 10, 20, 25, 30, 35, 40, 45},
	% yticklabel style={
	% 	/pgf/number format/precision=3,
	% 	/pgf/number format/fixed
	% },
	ymin=0,
	legend style={nodes={scale=0.8}},
	height=1.75in,
	width=2.0in,
	label style={font=\normalsize},
	title style={font=\large},
	tick label style={font=\tiny}
]


% gc graph 2
\nextgroupplot[ymax=75, ytick={0.0, 25, 50, 75}, ylabel={\% Individuals With $P_{\text{flip}}>0$}
, title={German Credit}, xlabel={Num. Ens. Models}]

\addplot[color=blue,mark=triangle*,blue] coordinates {
(1.0, 59)
(5.0, 29)
(10.0,25)
(15.0, 18)
(20, 16)
};

\addplot[color=green,mark=triangle*,green] coordinates {
(1.0, 25)
(5.0, 18)
(10.0, 12)
(15.0, 07)
(20, 06)
};



% \addplot[color=yellow, mark=triangle*,yellow] coordinates {
% (0.0, 65.9)
% (0.1, 41.9)
% (0.2, 18.5)
% (0.30000000000000004, 4.3)
% (0.4, 0.4)
% };


% adult graph 2
\nextgroupplot[ymax=10, ytick={0.0, 2, 04, 6, 8, 20 }, title={Adult}, xlabel={Num. Ens. Models}]

\addlegendimage{black, mark=triangle*}
\addlegendentry{RS}
\addlegendentry{LOO}

%\addlegendentry{Seed (L)}

\addplot[color=blue,mark=triangle*,blue] coordinates {
	(1.0, 8.878721570187653)
(5.0, 4.2702738545189314)
(10.0, 3.0037795902128506)
(15.0, 2.539619388634706)
(20.0, 2.1550295073271004)
};

\addplot[color=green,mark=triangle*,green] coordinates {
	(1.0, 6.252901001259864)
(5.0, 3.2623831310921024)
(10.0, 2.3406935879583583)
(15.0, 1.9362111265831178)
(20.0, 1.6245607055235065)
};



% \addplot[color=yellow,mark=triangle*,yellow] coordinates {
% 	(0.0, 0.48073735163450704)
% 	(0.1, 0.0)
% 	(0.2, 0.0)
% 	(0.30000000000000004, 0.0)
% 	(0.4, 0.0)

% };
% seizure graph 2
\nextgroupplot[ymax=10, ytick={0, 2, 4, 6, 8, 10}, title={Seizure},
%y_label={$E_x[IUF(h,\gamma,x)]$}, 
xlabel={Num. Ens. Models}]

\addplot[color=blue,mark=triangle*,blue] coordinates {
	(1.0, 6.0)
(5.0, 2.8)
(10.0, 2.1159420289855072)
(15.0, 1.536231884057971)
(20.0, 1.391304347826087)
};

\addplot[color=green,mark=triangle*,green] coordinates {
	(1.0, 6.0)
(5.0, 3)
(10.0, 2)
(15.0, 0)
(20.0, 0)
};


% \addplot[color=yellow,mark=triangle*,yellow] coordinates {
% 	(0.0, 1.7739130434782608)
% 	(0.1, 0.5217391304347827)
% 	(0.2, 0.0608695652173913)
% 	(0.30000000000000004, 0.0)
% 	(0.4, 0.0)


% };

% FMNIST graph 2
\nextgroupplot[ymax=15, ytick={5,10,15}, xtick={1, 5, 10, 15, 20}, title={FMNIST}, xlabel={Num. Ens. Models}]

\addplot[color=blue,mark=triangle*,blue] coordinates {
	(1.0, 11.28)
(5.0, 2.76)
(10.0, 2.87)
(15.0, 2.04)
(20.0, 1.77)
};

\addplot[color=green,mark=triangle*,green] coordinates {
(1.0, 5.58)
(5.0, 1.92)
(10.0, 2.51)
(15.0, 2.5)
(20.0, 2.71)
};


% \addplot[color=yellow,mark=triangle*,yellow] coordinates {
% 	(0.0, 0.0)
% (0.1, 0.0)
% (0.2, 0.0)
% (0.30000000000000004, 0.0)
% (0.4, 0.0)
% (0.5, 0.0)
% (0.6000000000000001, 0.0)
% (0.7000000000000001, 0.0)
% (0.8, 0.0)
% (0.9, 0.0)

% };

% TODOOOOOOOOO
\nextgroupplot[ymax=5, ytick={0.0, 1, 2,3,4,5}, title={Taiwanese}, xlabel={Num. Ens. Models}]
%deep base
\addplot[color=blue,mark=triangle*,blue] coordinates {
	(1.0, 0)
(5.0, 0)
(10.0, 0)
(15.0, 0)
(20.0, 0)
};

\addplot[color=green,mark=triangle*,green] coordinates {
(1.0, 3.0266666666666667)
(5.0, 2.0266666666666665)
(10.0, 1.2933333333333333)
(15.0, 1.2666666666666666)
(20.0, 1.0)
};



%lin seed
% \addplot[color=yellow, mark=triangle*,yellow] coordinates {
% (0.0, 65.9)
% (0.1, 41.9)
% (0.2, 18.5)
% (0.30000000000000004, 4.3)
% (0.4, 0.4)
% };

% TODOOOOOOOOO
\nextgroupplot[ymax=50, ytick={0, 25, 50}, title={Warfarin}, xlabel={Num. Ens. Models}]
%deep base
\addplot[color=blue,mark=triangle*,blue] coordinates {
	(1.0, 0)
(5.0, 0)
(10.0, 0)
(15.0, 0)
(20.0, 0)
};

\addplot[color=green,mark=triangle*,green] coordinates {
	(1.0, 0)
(5.0, 0)
(10.0, 0)
(15.0, 0)
(20.0, 0)
};

%lin seed
% \addplot[color=yellow, mark=triangle*,yellow] coordinates {
% (0.0, 65.9)
% (0.1, 41.9)
% (0.2, 18.5)
% (0.30000000000000004, 4.3)
% (0.4, 0.4)
% };

\end{groupplot}

%\legend{Deep, Linear, Adv., Smooth};

\end{tikzpicture}
%\end{document}

==> intro.tex <==
%!TEX root=paper.tex
\section{Introudction}~\label{sec:introduction}

% Deep Neural Networks (DNNs) are increasingly being integrated into important decision-making processes, from medical diagnosis~\cite{} to credit risk analysis~\cite{}. In several of these applications, it is necessary to generate explanations of a deployed model's decision: either for the model's user to understand the decision well enough to trust it, such as in a medical context; or it even may be legally required,  such as in a financial loan application context, in order for the decision recipient learn how to change their behavior in order to get a different outcome from the model in the future.

Deep Networks are increasingly being integrated into decision-making processes which require model explanations during model deployment, from medical diagnosis~\cite{} to credit risk analysis~\cite{}.
%hiring~\cite{}--- and are on the horizon for myriad more applications, such as credit risk analysis~\cite{}. 
%Many of these applications require that a deployed model generate explanations of its decisions---for example, it is legally required that rejected loan applicants will receive an explanation of their decision if requested. %Even if it is not legally mandated, it is increasingly considered necessary for models integrated in important decision systems, such as those in medicine, to return explanations as required as a part of their deployment in order to increase user trust and understanding~\cite{PWC}. 
\emph{Counterfactual explanations}~\cite{wachter2018counterfactual} %are a common and well-studied explanation method that 
are often put forth as a simple and intuitive method of explaining decisions in such high-stakes contexts~\cite{million_recourse_credit_papers}. A counterfactual explanation for an input $x$ is the nearest point $x'$ that produces a desired outcome $y'$ from a model.% (e.g., the nearest potential accepted loan application to a rejected loan application). 
Intuitively, these explanations are intended to answer the question, "Why did point $x$ not receive outcome $y'$?", either to give instructions for \emph{recourse}, i.e. how an individual can change their behavior to get a different model outcome, (e.g. in a loan application setting), or as a check to ensure a model's decision is well-justified (e.g. in a medical context). 

Counterfactual explanations are often accessed under the assumption that the decision system on which they will be used is static: that is, the model that \emph{creates} the explanation will be the \emph{same} model to which the loan applicant soliciting recourse re-applies. %, or that the doctor requiring an justification for a model's decision decides to trust. 
However, during real model deployments in high-stakes situations, models are not constant through time: there are often retrainings in result of small dataset updates, or fine-tunings to ensure consistent optimal behavior~\cite{pwc}.

Thus, in order for counterfactuals to be usable in practice, they must return the same desired outcome not only in the model that generates them, but in similar models created during deployment. If not, beyond rendering the counterfactual ineffective as an explanation, it jeapordizes recourse: a rejected loan applicant who matches the behavior of their accepted counterfactual example may be again rejected.
%then the counterfactual is potentially ineffective as a method of understanding the current model's decision process---and even more problematically, it jeapordizes recourse a rejected loan applicant who works hard to match the behavior of their counterfactual example may be again rejected.

%move other work up to the top right after the first sentence, and then talk about the gemoetric intuition that fails between deep models and other models?

In this paper, we investigate the consistency of counterfactuals between deep models with arbitrary differences that may occur during deployment, i.e. random seed and one-point changes in the training set. We demonstrate that some of the most commonly used counterfactual explanation methods for deep models either are highly inconsistent between models, or very costly, in that the distance between the input and the counterfactual is high. While recent work that has investigated this problem in simpler models~\cite{pawelcyk} has pointed to increasing counterfactual cost, i.e. the distance between an input point and its counterfactual, as a method of increasing consistency, we show that this is not a sufficiently reliable signal to guide the search for stable counterfactuals, especially in deep models (Section ~\ref{sec:invalidation}).

Instead, we show that \emph{a model's local Lipschitz continuity around the counterfactual} is a more reliable indicator of the counterfactual's stability. Intuitively, this is due to the fact that points with a low Lipschitz constant in the model are more difficult for models to change their prediction on during training, which we prove in Section ~\ref{sed:method}. Following this result, introduce \emph{Stable Neighbor Search} (SNS), which finds counterfactuals by searching for points with a low local Lipschitz constant in the generating model (Section~\ref{sec:method}). We empirically demonstrate that SNS which generates consistent counterfactuals while maintaining a low cost relative to other methods. 

%Recent work has investigated this problem of counterfactual inconsistency~\cite{pmlr-v124-pawelczyk20a}, but solely in models with strongly calibrated predictions. Other recent work~\cite{rawal2021i} has addressed a related problem, namely stability of counterfactual explanations across large-scale \emph{distribution shifts} between models, i.e. models retrained an an entirely new, but similar dataset. Arguably, however, such large changes may require invalidation, as the model must learn something new from a substantial change in its data distribution. 

%Recent work has demonstrated that higher cost counterfactuals, i.e. those farther away from the input that requires an explanation, are more likely to remain consistent between the linear and other well-calibrated models that they consider. In a linear model, this intuition makes sense: the farther away a point is across a boundary from a point of the opposite class, the less likely the point will be affected by small perturbations to that boundary. 

%However, in a deep model with a highly complex network of boundaries, going farther away from a point across the nearest boundary may in fact lead to being closer to a different boundary. Thus, as we empirically demonstrate (Section~\ref{sec:invalidation}), increasing a counterfactual's cost is does not guarantee higher consistency between nearby models. While higher than minimal cost is necessary to achieve a consistent counterfactual, previous work gives little sense of to navigate the trade-off between cost and consistency. As we later demonstrate (Section ~\ref{sec:evaluation}), our method, Robust Neighbor Search provides a principled way to generate consistent counterfactuals at a lower cost (less than half) than solutions recommended by previous work.
%Thus, as we empirically demonstrate~\ref{sec:evaluation}, naively increasing a counterfactual's cost as a method of increasing consistency between nearby models can either be ineffective, or lead to counterfactuals with extremely high costs.  

%Understanding how RNS achieves this requires considering deep model geometry. Intuitively, RNS hinges on the theoretical observation that points with a low Lipschitz constant in the model are more difficult for models to change their prediction on during training (Section ~\ref{sed:method}). %This is due to the fact that, from the perspective of the loss, these points incur a high cost to move between classes. 
%This suggests that they the outcome of such points will be more consistent between models with small differences, as they optimize the same loss. Following this intuition, we prove that RNS finds counterfactuals by searching for points with a low local Lipschitz constant in the generating model (Section~\ref{sec:method}).%, and finally, empirically demonstrate its ability to find stable counterfactuals at a relatively low cost compared to other methods (Section~\ref{sec:evaluation}). 

In summary, our main \textbf{contributions} are: 1) We demonstrate that common counterfactual explanations can have low consistency across nearby \emph{deep} models, and that cost is an insufficient signal to find consistent counterfactuals; 2) To more optimally navigate this cost-consistency tradeoff, we prove that counterfactual examples in a neighborhood where the network has low local Lipschitz Constant are more consistent against small changes in the training environment (Theorem.~\ref{theorem:loss-and-lipschitz}); 3) Leveraging this result, we propose \emph{Stable Neighbor Search} (RNS) as a way to generate consistent counterfactual explanations (Def.~\ref{def:RNS}); 4) We empirically demonstrate the effectiveness RNS in generating consistent and low-cost counterfactual explanations.


%__old intro 2---

% Deep Networks are increasingly being integrated into decision-making processes which require model explanations during model deployment, from medical diagnosis~\cite{} to credit risk analysis~\cite{}.
% \emph{Counterfactual explanations}~\cite{wachter2018counterfactual} 
% are often put forth as a simple and intuitive method of explaining decisions in such high-stakes contexts~\cite{million_recourse_credit_papers}. A counterfactual explanation for an input $x$ is the nearest point $x'$ that produces a desired outcome $y'$ from a model.
% Intuitively, these explanations are intended to answer the question, "Why did point $x$ not receive outcome $y'$?", either to give instructions for \emph{recourse}, i.e. how an individual can change their behavior to get a different model outcome, (e.g. in a loan application setting), or as a check to ensure a model's decision is well-justified (e.g. in a medical context). 

% Counterfactual explanations are often accessed under the assumption that the decision system on which they will be used is static: that is, the model that \emph{creates} the explanation will be the \emph{same} model to which the loan applicant soliciting recourse re-applies. %, or that the doctor requiring an justification for a model's decision decides to trust. 
% However, during real model deployments in high-stakes situations, models are not constant through time: there are often retrainings in result of small dataset updates, or fine-tunings to ensure consistent optimal behavior~\cite{pwc}.

% Thus, in order for counterfactuals to be usable in practice, they must return the same desired outcome not only in the model that generates them, but in similar models created during deployment. If not, beyond rendering the counterfactual ineffective as an explanation, it jeapordizes recourse: a rejected loan applicant who matches the behavior of their accepted counterfactual example may be again rejected.
% %then the counterfactual is potentially ineffective as a method of understanding the current model's decision process---and even more problematically, it jeapordizes recourse a rejected loan applicant who works hard to match the behavior of their counterfactual example may be again rejected.

% %move other work up to the top right after the first sentence, and then talk about the gemoetric intuition that fails between deep models and other models?

% % In this paper, we investigate the consistency of counterfactuals between deep models with arbitrary differences that may occur during deployment, i.e. random seed and one-point changes in the training set. We demonstrate that some of the most commonly used counterfactual explanation methods for deep models either are highly inconsistent between models, or very costly, in that the distance between the input and the counterfactual is high. To mitigate the problem of counterfactual inconsistency in deep models, we introduce a new method of counterfactual generation, \emph{Robust Neighbor Search} (RNS), which generates consistent counterfactuals at while maintaining a low cost relative to other methods. 

% %Recent work has investigated this problem of counterfactual inconsistency~\cite{pmlr-v124-pawelczyk20a}, but solely in models with strongly calibrated predictions. Other recent work~\cite{rawal2021i} has addressed a related problem, namely stability of counterfactual explanations across large-scale \emph{distribution shifts} between models, i.e. models retrained an an entirely new, but similar dataset. Arguably, however, such large changes may require invalidation, as the model must learn something new from a substantial change in its data distribution. 

% Recent work has demonstrated that higher cost counterfactuals, i.e. those farther away from the input that requires an explanation, are more likely to remain consistent between the linear and other well-calibrated models that they consider. In a linear model, this intuition makes sense: the farther away a point is across a boundary from a point of the opposite class, the less likely the point will be affected by small perturbations to that boundary. 

% However, in a deep model with a highly complex network of boundaries, going farther away from a point across the nearest boundary may in fact lead to being closer to a different boundary. Thus, as we empirically demonstrate (Section~\ref{sec:invalidation}), increasing a counterfactual's cost is does not guarantee higher consistency between nearby models. While higher than minimal cost is necessary to achieve a consistent counterfactual, previous work gives little sense of to navigate the trade-off between cost and consistency. As we later demonstrate (Section ~\ref{sec:evaluation}), our method, Robust Neighbor Search provides a principled way to generate consistent counterfactuals at a lower cost (less than half) than solutions recommended by previous work.
% %Thus, as we empirically demonstrate~\ref{sec:evaluation}, naively increasing a counterfactual's cost as a method of increasing consistency between nearby models can either be ineffective, or lead to counterfactuals with extremely high costs.  

% Understanding how RNS achieves this requires considering deep model geometry. Intuitively, RNS hinges on the theoretical observation that points with a low Lipschitz constant in the model are more difficult for models to change their prediction on during training (Section ~\ref{sed:method}). %This is due to the fact that, from the perspective of the loss, these points incur a high cost to move between classes. 
% This suggests that they the outcome of such points will be more consistent between models with small differences, as they optimize the same loss. Following this intuition, we prove that RNS finds counterfactuals by searching for points with a low local Lipschitz constant in the generating model (Section~\ref{sec:method}).%, and finally, empirically demonstrate its ability to find stable counterfactuals at a relatively low cost compared to other methods (Section~\ref{sec:evaluation}). 

% In summary, our main \textbf{contributions} are: 1) We demonstrate that common counterfactual explanations can have low consistency across nearby \emph{deep} models, and that cost is an insufficient signal to find consistent counterfactuals; 2) To more optimally navigate this cost-consistency tradeoff, we prove that counterfactual examples in a neighborhood where the network has low local Lipschitz Constant are more consistent against small changes in the training environment (Theorem.~\ref{theorem:loss-and-lipschitz}); 3) Leveraging this result, we propose \emph{Robust Neighbor Search} (RNS) as a way to generate consistent counterfactual explanations (Def.~\ref{def:RNS}); 4) We empirically demonstrate the effectiveness RNS in generating consistent and low-cost counterfactual explanations.

%__OLD INTRO 1__
% Deep networks are increasingly being integrated into important decision-making processes, from medical diagnosis~\cite{} to credit risk analysis~\cite{}. In several of these applications, it is necessary to generate explanations of a deployed model's decision: either for the model's user to understand the decision well enough to trust it, such as in a medical context; or it may be legally required,  such as in a financial loan application context, in order for the decision recipient learn how to change their behavior in order to get a different outcome from the model in the future.

% One common explanation method used in a variety of contexts is a \emph{counterfactual} explanation~\cite{wachter2018counterfactual}, which, given an input and a model, returns a nearby input that is classified as the opposite class. These explanations are used in a variety of applications as they are quite easy to understand and can be generated for any kind of model.

% In order for explanations to be useful, however, they must work--that is, if a person who applied for a loan and was rejected by a deep learning model does reapply, and changes their behavior to match the counterfactual shown to them as a guarantee of approval, they should have their loan approved. Similarly, if a doctor investigates a model's decision via a counterfactual explanation and decides it is sound, the model should not inexplicably change its behavior on that counterfactual, as it may change the doctor's view of the model's reasoning.

% Counterfactuals are often generated and evaluated under the assumption that the underlying model that generates and evaluates these counterfactuals does not change. However, when machine learning models are used in important deployment contexts, they are often periodically retrained to ensure continued performance. Thus, in deployment, models are not quite constant, but often go through small changes as a result of these quality control processes. %in order for explanations to be useful, 
% Consequently, explanations must be invariant to inconsequential changes to the model, that may arise from this process---for example changing the random seed, or small differences in the training set. 

% In this paper, we show that commonly used counterfactual explanation methods are not invariant to these small changes. That is, a counterfactual produced in one model will
% likely not produce the same desired output in another model with a small arbitrary change e.g. to random seed or the training set. We call this behavior counterfactual invalidation, and we show that it can happen up to 96\% of the time. Beyond this, intuitive changes to the counterfactual generation process that may prevent invalidation, e.g. requiring that counterfactuals have high confidence in the generating model, prove to be largely ineffective at reducing invalidation. While we do see some counterfactual generation methods have lower invalidation percentages, such as those that attempt to generate counterfactuals within the data manifold, it remains unacceptably high (~10\%), and the examples generated are often extremely costly, potentially making them intractable for a real user in the case of recourse.

% We prove that using models trained to have a low Lipschitz constant generate counterfactuals with lower invalidation rates than unconstrained models, and empirically demonstrate that this holds in practice. However, the extent to which using Lipschitz models alone does not always satisfactorily solve the problem in practice, and they too often generate higher-cost counterfactuals. To further ameliorate this problem, we introduce a new counterfacutual generation method, robust neighbor search (RNS), which generates counterfactuals stable to arbitrary changes at a low cost, and empirically demonstrate its effectiveness.


%We show that commonly used counterfactual explanation methods are unstable across deep models with similar accuracy, and arbitrary differences such as random seed or a one-point difference in the training set. 



%Specifically, hig their method of finding equivalent models relies on changing hyperparameters or hypothesis class, which 

% Other work has investigated counterfactual invalidation in the presence of larger-scale distribution shift~\cite{rawal2021i}, i.e. retraining on a substantially modified dataset, e.g. the same features collected in two different countries. In this situation, some invalidation of counterfactual examples may even be expected as the model may shift its predictions in response to new information. They prove that a tradeoff exists between the cost of a counterfactual 









% Contributions:



% - We demonstrate the extent of inconsistency of counterfactual explanations between similar deep models with \emph{arbitrary} differences in training environment, such as random seed or one-point difference in the training set. We show that some common sense intuitions on how to lower invalidation rate do not hold sufficiently well in deep models to mitigate this problem: namely, generating higher confidence counterfactuals, and generating higher cost counterfactuals.

% - We prove that models with a bounded Lipschitz constant will have lower counterfactual invalidation than unbounded models.
% - We empirically verify our result with experiments showing decreased invalidation of counterfactual examples between models with low lipschitz constants.
% - We provide a new counterfactual search method, robust neighbor search (RNS), that generated counterfactuals at a lower cost with a low invalidation rate while maintaining a low cost.



% Background and Preliminaries 





==> lipschitz.tex <==
% !TEX ROOT=./neurips_2021.tex

Characterizing the precise effect that changes such as random initialization have on the outcome of training is challenging. 
We approach this by modeling the differences that arise from small changes as a \emph{refinement} of the original model. 
We assume that a model $F(\xvec;\theta^{(k)}), k > 0$ can be derived from a \emph{generating} model $F(\xvec;\theta^{(0)})$ by applying some finite number of gradient descent updates to get $\theta^{(k)} \leftarrow \theta^{(0)}$. 
Within this framework, we proceed to show that given a counterfactual $\xvec_c$ for $\xvec$, the local Lipschitz constant of $F(\xvec;\theta^{(0)})$ at $\xvec_c$ serves as a proxy for the difficulty of invalidating $\xvec_c$ through refinement.
Our main supporting result is given in Theorem~\ref{theorem:loss-and-lipschitz}, which shows that wherever the model is locally-Lipschitz, the loss must be large to invalidate $\xvec_c$ through refinement.
Lemma~\ref{lemma:loss-and-lipschitz} bounds the gradient norm of the loss at such points, and follows as a natural consequence.

\begin{theorem}\label{theorem:loss-and-lipschitz}
	Let $F(\xvec;\theta^{(i)})$ be a network with a single logit output (i.e., a binary classifier) that is $(K, \epsilon)$-locally Lipschitz at $\xvec$. 
	If $\epsilon$ is greater than the distance between $\xvec$ and the closest decision boundary in $F$, then for $y \in \{0,1\}$, $||\nabla_\theta \mathcal{J}(\xvec, 1-y)||_2 \leq (1-(1+\exp(K\epsilon))^{-1})\cdot ||\nabla_{\theta^{(i)}} f(\xvec, \theta^{(i)})||_2$
	% \begin{align*}
	% 	\mathit{1)}\ F(\xvec;\theta^{(i)}) = F(\xvec;\theta^{(i+1)})
	% 	&&
	% 	\mathit{2)}\ \mathcal{J}(\xvec, 1-y) \geq -\log(1+\exp(K\delta))
	% \end{align*}
	% \begin{align*}
	%  \mathcal{J}(\xvec, 1-y) \geq -\log(1+\exp(K\delta))
	% \end{align*}
	where $\mathcal{J}$ is the cross-entropy loss and $y$ is the label for $\xvec$.
\end{theorem}

\begin{corollary}\label{lemma:loss-and-lipschitz}
	Let $F(\xvec;\theta^{(i)})$, $\xvec_1$ and $\xvec_2$ be a network and two points as described in Theorem~\ref{theorem:loss-and-lipschitz}, if $F$ is $(K_1, \epsilon)$-locally Lipschitz at $\xvec_1$ and $(K_2, \epsilon)$-locally Lipschitz at $\xvec_2$ and $K_1 \leq K_2$, then with all hyperparameters identical in refining the network $\theta^{(i+1)} \leftarrow \theta^{(i)}$, it takes more steps to flip the prediction on $\xvec_1$ than it does to flip the prediction on $\xvec_2$.
	
	% when using SGD to minimize the Cross Entropy loss to flip the prediction of $\xvec$, in the first iteration, $||\nabla_\theta \mathcal{J}||_2 \leq (1-1/(1+\exp(K\delta))\cdot ||\nabla_{\theta} f||_2$.
\end{corollary}

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/surface_bump.png}
        \caption{}
        \label{fig:illustration-surface}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{images/circle.png}
        \caption{}
        \label{fig:illustration-circle}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{images/curve.png}
        \caption{}
        \label{fig:illustration-curve}
     \end{subfigure}
    \caption{(a) A visual illustration for the intuition behind Theorem \ref{theorem:loss-and-lipschitz}. Point A and B are counterfactuals on the same side of the decision boundary $D$. Smaller local Lipschitz Constant of the model's output indicates a more flattened neighborhood for point B; therefore counterfactual $B$ is more consistent than point A. (b) a visual illustration shows how Eq.~(\ref{Eq:find_robust_neighbor-challenge-one}) is approximated with Eq.~(\ref{Eq:find_robust_neighbor-challenge-two}) by only considering points on a line segment $t\in[a, 1]$. (c) the curve of the model's output $f(r(t\hat{\xvec};\theta))$ against $t$.}
 \end{figure}

A visual illustration of the main insight in Theorem~\ref{theorem:loss-and-lipschitz} is shown in Fig.~\ref{fig:illustration-surface}. The counterfactual $B$, which resides in a flatter, more locally-Lipschitz region of the decision surface, would need a greater loss than $A$, which resides in a steeper region that will have corresponding loss gradients whose norms are larger.
Specifically, Theorem~\ref{theorem:loss-and-lipschitz} indicates that the more Lipschitz continuous $F(\xvec_c;\theta^{(0)})$ is at $\xvec_c$, the more any refinement $F(\xvec_c;\theta^{(k)})$ will need to minimize the loss around $\xvec_c$ to effect its invalidation.
In addition, Lemma~\ref{lemma:loss-and-lipschitz} shows that in the first iteration of parameter update using a method like SGD, the gradient norm of the loss at $\xvec_c$ decreases inversely to its Lipschitz continuity, and thus, the magnitude of the update will be smaller. 
Accordingly, for fixed number of iterations and learning rate, the initial loss and gradient make it hard for refinement to invalidate counterfactuals with small local Lipschitz constants.

Although Theorem~\ref{theorem:loss-and-lipschitz} does not provide a general answer to the question of how likely it is that a counterfactual will be invalidated in a closely-related network, it characterizes the difficulty of invalidating a point through subsequent training updates, and the conditions that are salient to such an outcome. 
Interestingly, it also explains why counterfactuals with high cost, even if they are predicted confidently by the network or far from a decision boundary, may still be invalidated as we saw in Figure~\ref{fig:toy-non-linear}: if it resides in a less locally-Lipschitz region, then the magnitude of the updates on nearby training points may be great enough to cause invalidation.


==> other_Scrap.tex <==

\section{Related Work}\label{sec:related-work-2}
This work focuses on evaluating and improving the consistency of prediction of counterfactual examples across duplicitous deep models, with inconsequential differences in the training set. 
While counterfactual examples ...., recent work has also pointed to problems with counterfactuals examples~\cite{laugel2019issues,}.

Counterfactual examples are a popular explanation method, often suggested for use in contexts legally requiring an explanation, for example for industries impacted by the \emph{General Data Protection Regulation} (GDPR). As mentioned earlier, there is much research work devoted to finding methods of finding the most actionable, realistic, explanatory, causally motivated, or otherwise optimal counterfactual~\cite{verma2020counterfactual,sokol2019counterfactual,wachter2018counterfactual,keane2020good,dandl2020multi,pawelczyk2020learning}. Despite their popularity, recent work has also pointed to problems with counterfactuals examples~\cite{laugel2019issues}. Beyond works pointing out counterfactual instability across duplicitous models~\cite{pmlr-v124-pawelczyk20a}, and across large-scale distribution shifts~\cite{rawal2021i}, Barocas et al.~\cite{barocas2016big},  points to the tension between the usefulness of a counterfactual and the ability to keep the explained model private, and the possibility of a counterfactual giving bad advice in a global sense (e.g. taking on more debt), even if it is valid advice to get a desired outcome from a model. 
%models beyond instability~\cite{barocas2016big,laugel2019issues}. For example, Barocas et al~\cite{barocas2016big},  also points to the tension between the usefulness of a counterfactual and the ability to keep the explained model private.

%Pawelczyk et al. built on these prior works by evaluating the consistency of counterfactual examples across similar models, although they restrict their analysis to highly calibrated models\cite{pmlr-v124-pawelczyk20a}. They, along with other work that investigates counterfactual inconsistency across large scale distribution shifts~\cite{rawal2021i}, show that higher-cost counterfactuals are less likely to be invalidated than lower-cost counterfactuals in linear, or well-calibrated models. In this paper, we focus on evaluating the problem of counterfactual inconsistency in deep models, where this assumption of calibration does not hold. Further, unlike other recent work, introduce a counterfactual generation method, Stable Neighbor Search, designed to specifically target consistent counterfactuals in deep models, that reaches low invalidation while keeping a relatively low cost. 

%Interestingly, Pawelczyk et al. demonstrate that counterfactuals drawn from the data distribution tend to have lower invalidation rates than minimum-cost counterfactuals, which we also show can hold true in deep models--though Stable Neighbor Search can lower the invalidation further. While they suggest the higher cost of data-based counterfactuals ,as a potential reason for this, our theoretical results point to another intuitive reason: following intuition from Theorem ~\ref{theorem:loss-and-lipschitz}, a model's boundaries are likely to be more stable on points in the training set, as changing prediction on these points incurs a high cost from the perspective of the loss. As points in the data distribution are going to be closer to regions around points in the training set, choosing counterfactuals from the data distribution may be akin to choosing counterfactuals from regions of the decision space where the boundary changes less drastically.

%They, along with other work that investigates counterfactual inconsistency across large scale distribution shifts~\cite{rawal2021i}, show that higher-cost counterfactuals are less likely to be invalidated than lower-cost counterfactuals in linear, or well-calibrated models. In this paper, we focus on evaluating the problem of counterfactual inconsistency in deep models, where this assumption of calibraton does not hold. Further, unlike prior work, we introduce a method to mitigate counterfactual inconsistency in deep models that reaches low invalidation while keeping a relatively low cost.
%Recent work has shown that duplicitious models,

% While in this work, we demonstrate and address the problem of duplicitous deep models producing varying outputs on \emph{counterfactual examples}, recent work has shown that, more broadly, there are large differences between model prediction behavior on ~\emph{any} input across small changes to the model, not specifically counterfactual examples~\cite{blackleave2021,marx2019,mehrer2020individual}. Instability has also been shown to be a problem for a broader class of explanations methods, such as gradient-based explanations, although this is largely studied in an adversarial context~\cite{dombrowski2019explanations,ghorbani2019interpretation,heo2019fooling}.

Adversarial examples~\cite{Goodfellow2015ExplainingAH} more broadly have long been known to be a mathematically similar to counterfactual examples, used in essentially opposite contexts. Within work on adversarial examples, there is a recent interest of \emph{adversarial transferability}~\cite{dong2018boosting,ilyas2019adversarialnotbugs,Xie_2019_CVPR}, where adversarial attacks are induced to transfer between models. However, adversarial transferability concerns itself with transferring attacks between extremely different models in different contexts--e.g., trained on disjoint training sets, or with completely different architectures---or even without knowledge of the model to which attacks are to be transferred. Meanwhile, in this work, we work on decreasing invalidation to near zero between very \emph{similar} models, in order to ensure consistency of counterfactual examples, to preserve recourse in a deployment setting with frequent re-trainings. We look forward to exploring the potential overlap between these two areas of research as promising future work. 
%Some of these papers point to the fact that this problem is especially bad on out-of-distribution points~\cite{googlepaper}, again pointing to the 
%However, unlike Marx et al., we only consider changes to the model that are do not affect the model's optimization function. Specifically, we restrict our search of nearby models to those only differing in the random initialization and small changes to the training set, instead of searching over hyper-parameters.

% Recent work has shown that there are large differences between model prediction behavior on ~\emph{any} input across small changes to the model, not specifically counterfactual examples~\cite{blackleave2021,flavio,google_paper}. We, along with Marx et al. (and Pawelczyk et al.)~\cite{flavio}, restrict the models we evaluate consistency over to be within a certain accuracy bound of a trained baseline model. However, unlike Marx et al. and Pawelczyk et al, we only consider changes to the model that are "arbitrary" in that they do not affect the model's optimization function. Specifically, we restrict our search of nearby models to those only differing in the random initialization and small changes to the training set, instead of searching over hyperparameters.


==> other_method_section_git_mishap.tex <==
% !TEX ROOT=./neurips_2021.tex
\section{Counterfactual Invalidation in Deep Models}\label{sec:invalidation}

As we demonstrate in more detail in Section ~\ref{sec:evaluation}, counterfactual invalidation is a problem in deep networks on real data: counterfactuals produce inconsistent outcomes in duplicitous deep models up to 94\% of the time. 

Previous work investigating the problem of counterfactual invalidation~\cite{pmlr-v124-pawelczyk20a,rawal2021i}, has pointed to increasing counterfactual cost as a potential mitigation strategy.
%Previous work has pointed out the relationship between counterfactual cost and invalidation rate, 
In particular, they prove that higher cost counterfactuals will lead to lower invalidation rates in linear models in expectation~\cite{rawal2021i}, and demonstrate their relationship in a broader class of well-calibrated models~\cite{pmlr-v124-pawelczyk20a}. While this insight provides interesting challenge to the perspective that low cost counterfactuals should be preferred, we show that cost alone is insufficient to determine which counterfactual has a greater chance of being consistent at generation time in deep models.

The intuition that a larger distance between input and counterfactual will lead to lower invalidation rests on the assumption that the distance between a point $x$ and a counterfactual $x_c$ is indicative of the distance from $x_c$ from the decision boundary, with a higher distance making $x_c$'s prediction more stable under small perturbations to that boundary. This holds well in a linear model, where there is only one boundary~\cite{rawal2021i}. 

However, in the complex decision boundaries of deep networks, going farther away from a point across the \emph{nearest} boundary may lead to being closer to a \emph{different} boundary. We prove that this holds even for a one-hidden-layer network by Theorem~\ref{theorem:cost-in-deep-models}. This observation shows that a counterfactual example that is farther from its origin point may be equally susceptible to invalidation as one closer to it. In fact, we show that the \emph{only} models where $\ell_p$ cost is universally a good heuristic for distance from a decision boundary, and therefore by the reasoning above, consistency, are linear models (Lemma~\ref{lemma:cost-in-deep-models}). 

\begin{theorem}\label{theorem:cost-in-deep-models}
Suppose that $H_1, H_2$ are decision boundaries in a piecewise-linear network $F(\xvec) = sign\{w_1^\top ReLU(W_0\xvec)\}$, and let $\xvec$ be an arbitrary point in its domain. 
If the projections of $\xvec$ onto the corresponding halfspace constraints of $H_1, H_2$ are on $H_1$ and $H_2$, then there exists a point $\xvec'$ such that:
\begin{align*}
\mathit{1)}\ d(\xvec', H_2) = 0 & &
\mathit{2)}\ d(\xvec', H_2) < d(\xvec, H_2) & &
\mathit{3)}\ d(\xvec, H_1) \leq d(\xvec', H_1)
\end{align*}
where $d(\xvec, H_*)$ denotes the distance between $\xvec$ and the nearest point on a boundary $H_*$.
\end{theorem}
    
\begin{lemma}\label{lemma:cost-in-deep-models}
Let $H_1, H_2, F$ and $\xvec$ be defined as in Theorem~\ref{theorem:cost-in-deep-models}. 
If the projections of $\xvec$ onto the corresponding halfspace constraints of $H_1, H_2$ are on $H_1$ and $H_2$, but there \emph{does not} exist a point $\xvec'$ satisfying \emph{(2)} and \emph{(3)} from Theorem~\ref{theorem:cost-in-deep-models}, then $H_1$ = $H_2$.
\end{lemma}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.29\textwidth}

        \includegraphics[width=\textwidth]{images/toy_data.png}
        \caption{}
        \label{fig:toy-data}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}

        \includegraphics[width=\textwidth]{images/toy_non_linear.png}
        \caption{}
        \label{fig:toy-non-linear}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{images/toy_linear.png}
        \caption{}
        \label{fig:toy-linear}
     \end{subfigure}
    \caption{Illustration of the boundary change in a deep model (b) and a linear model (c) for a 2D dataset (a) when changing the seed for random initialization during the training. Shaded regions correspond to the area when two deep models in (b) (or two linear models in (c)) make different predictions.}
    \label{fig:cost-intuition}
 \end{figure}


% \begin{proof}
% We prove this lemma by demonstration. Consider the deep model in Figure ~\ref{fig:lemma_pic}. See that for point $x_1$, the higher-cost counterfactual generated for that point in the is actually closer to the decision boundary than the lower-cost counterfactual.
% \end{proof}

%While Theorem~\ref{theorem:cost-in-deep-models} and Lemma~\ref{lemma:loss-and-lipschitz} are constrained in one-layer models, the insights generalize to more complicated models. 
Figure~\ref{fig:cost-intuition} illustrates the geometric intuition behind these results. 
The shaded regions of ~\ref{fig:toy-non-linear} correspond to two decision surfaces trained from different random seeds on the data in (a).
The lighter gray region denotes where the models disagree, whereas the black and white regions denote agreement.
Observe that counterfactuals equally far from a decision boundary may have different invalidation behavior, as demonstrated by the counterfactuals $c_1$ and $c_2$ for the point $x_2$.
Also note that as shown with $x_1$, being far away from one boundary may lead one to cross another one in deep models. 
However, for two linear models shown in Fig.~\ref{fig:toy-linear}, being far away from the boundary is indeed a good indicator or being consistent.


The discussion so far has demonstrated that there is not a strong theoretical relationship between cost and invalidation in deep models. 
Later in Section ~\ref{sec:evaluation}, we test this claim on real data, and show that higher-cost counterfactuals in some cases have \emph{higher} invalidation rates than their lower-cost relatives (c.f. Table~\ref{table_IV}). 
Further, we show that the coefficient of determination ($R^2$) between cost and invalidation rate is very
%exceedingly
 small (with all but one around 0.05). 

Thus, while cost and invalidation are certainly related---for example, it may be necessary for a stable counterfactual to be more costly than the \emph{minimum} point across the boundary---cost alone is not enough to determine which one will be the most consistent in deep models. 
% In the next section, we show the local Lipschitz continuity of a point serves as a reliable signal to find stable counterfactuals in deep models.

\section{Towards Consistent Counterfactuals}
\label{sec:method}
In this section, we first demonstrate that the local Lipschitz Condition (Def.~\ref{def:local-lipschitz-continuity}), can be leveraged to characterize the consistency of counterfactual explanations under changes to the network's parameters (Section~\ref{sec:lipschitz}). 
We further discuss insights from these analytical results and introduce an effective approach, \emph{Stable Neighbor Search}, to improve the consistency of counterfactual explanations (Section~\ref{sec:sns}).
Unless otherwise noted, this section assumes all norms are $\ell_2$.

\begin{definition}[Local Lipschitz Continuity]\label{def:local-lipschitz-continuity}
    A function $h:\mathbb{R}^d \rightarrow \mathbb{R}$ is \emph{$(K, \epsilon)$-locally Lipschitz continuous at $\xvec$} iff $\forall \xvec' \in B(\xvec, \epsilon) . |h(\xvec') - h(\xvec)| \leq K ||\xvec'-\xvec||$. 
    We refer to $K$ as the \emph{local Lipschitz constant} of $h$ at $\xvec$.
\end{definition}

\subsection{Local Lipschitz Continuity and Consistency}
\label{sec:lipschitz}
\input{lipschitz}

\subsection{Finding Consistent Counterfactuals}
\label{sec:sns}
\label{RNS}
\input{RNS}

% \subsection{Lipschitz Network}
% \input{lip_network}

==> proof_draft.tex <==
%!TEX root=paper.tex


\begin{proposition}
Consider a binary classification model $H : R^n \rightarrow \{0,1\} = \text{sign}(h)$, where $h: R^n \rightarrow R$. Given an arbitrary function $g: R^n \rightarrow R$ which is bounded from above and below, continuous, and piece-wise differentiable, and a constant $\epsilon < 0$, it is possible to construct a model $\hat{H} : R^n \rightarrow \{0,1\} = \text{sign}(\hat{h})$, $\hat{h}: R^n \rightarrow R$, where the gradients of $\hat{h}$ are determined by this arbitrary function $g$, except within $\frac{\epsilon}{2}$ of a decision boundary, but where $H(x)=\hat{H}(x) \forall x$. That is, the thresholded classification behavior is the same for both models $H$ and $\hat{H}$, but their underlying functions $h$ and $\hat{h}$ have arbitrarily different gradients, and therefore arbitrarily different gradient-based explanations, almost everywhere. %maintains the same mapping $\hat{H}: R^n \rightarrow \{0,1\} = h: S \rightarrow \{0,1\}$.
%Specifically, this means that $h$ and $\hat{h}$ will have the same 0/1 loss and prediction behavior as $h$, but arbitrarily different gradient-based explanations. 
\end{proposition}
\begin{proof}
We divide $R^n$ into regions $\{I_1....I_k\}$ determined by the decision boundaries of $H$. That is, each $I_i$ represents an area where $H$ predicts a certain class ($-1$ or $1$) up until the boundaries to predict a different class.
%We are given a function $g$, which we divide into functions $g_i(x): x \in I_i \rightarrow R$, i.e. we divide the range of $g$ to create functions that are specific to each decision region $\{I_1....I_k\}$ of $H$. 

%Then, we create a set of functions $\hat{g_{I_i}}(x): x \in I_i \rightarrow R$ such that
Recall we are given a function $g: R^n \rightarrow R$ which is bounded from above and below. We create a set of functions $\hat{g_{I_i}}(x): x \in I_i \rightarrow R$ such that 
\[
\hat{g}_{I_i}(x)= \begin{cases} 
g(x)-\inf_x g(x)   \text{    if $H(I_i)=1$} \\
g(x)-(\sup_x g(x) + c) \text{    if $H(I_i)=-1$}
\end{cases}
\]%Consider the function $\hat{g}= g_i(x)$ for $x \in I_i$. 

Where $c$ is some constant greater than zero. Additionally, let $d(x)$ be the $\ell_2$ distance from $x$ to the nearest decision boundary of $h$. Then, we define $\hat{h}$ to be:

\[ \hat{h} =  \begin{cases}
\hat{g}_{I_i}(x) \text{ for x } \in I_i \text{ if $d(x) > \frac{\epsilon}{2}$}\\
\hat{g}_{I_i}(x) \times \frac{2d(x)}{\epsilon} \text{ for x } \in I_i \text{ if $d(x) \leq \frac{\epsilon}{2}$} \\
\end{cases}
\]

And, as described above, we define $\hat{H}=\text{sign}(h)$. 
First, we show that $\hat{H}(x)=H(x) \forall x \in R^n$.
Consider the case when $H(x)=1$, and $d(x)> \frac{\epsilon}{2}$. 
By construction, $\hat{H}(x)= \text{sign}(h(x))= \text{sign}(\hat{g}_{I_i}(x)) = \text{sign}(g(x)-\inf_x g(x))$, where $x \in $ region $I_i$ where $H(I_i)=1$. By definition of the infimum, $g(x)-\inf_x g(x)>=0$, and thus $\text{sign}(g(x)-\inf_x g(x))=1$, and $\hat{H}(x)=1=H(x)$.
Note that in the case where $d(x) \leq \frac{\epsilon}{2}$, we can follow the same argument as the value of $\hat{h(x)}$ only differs by a positive constant. A similar argument follows for the case where $H(x)=-1$; thus, $\hat{H}(x)=H(x) \forall x \in R^n$.

Secondly, we show that $\bigtriangledown \hat{h}(x)= \bigtriangledown g(x) \forall x \text{where} d(x) > \frac{\epsilon}{2}$. Consider the case where $H(x)=1$.
By construction, $\hat{h}(x)=\hat{g}_{I_i}(x)= g(x)-\inf_x g(x)$. Note that this means $\hat{h}(x)=g(x)$ plus a constant, so the gradient of the two functions at $x$ is the same. A symmetric argument holds for the case where $H(x)=-1$.

%Note that this construction necessitates that $\hat{h}(x)=0$ if and only if $h(x)=0$, as $g_i(x)-\inf_x g_i(x)>0$, and $\hat{g}(x)$ is defined this way when $h(x)=0$. Similarly, $\hat{g}(x)=1$ if and only if $h(x)=1$. Further, see that $\bigtriangledown \hat{g}(x)= \bigtriangledown g(x) \forall x \text{where} d(x) < \epsilon$, as $\hat{g_i}(x)$ and $g_i(x)$ only differ by a constant for all $i$, and thus the gradient must be the same.   


It remains to prove that $\hat{h}$ is continuous and piece-wise differentiable, in order to be a realizable as a Relu-network. See that $\hat{h}$ is piece-wise differentiable as $g$ is, as required, which means that $\hat{g_i}$ are continuous well, and also $\hat{g_i}(x) \times \frac{d(x)}{\epsilon} \forall i$, which comprise $\hat{h}$. To see that $\hat{h}$ is continuous, consider the case where $d(x)=\epsilon$ for some x: then $\hat{g_i}(x) \times \frac{d(x)}{\epsilon} = \hat{g_i}(x) \times \frac{\epsilon}{\epsilon}= \hat{g_i}(x)$. Additionally, consider the case where $d(x)=0$, i.e. $x$ is on a decision boundary of $h(x)$, between two regions $I_i, I_j$. Then $\hat{h}(x)=\hat{g_i}(x) \times \frac{d(x)}{\epsilon}= \hat{g_i}(x) \times 0= 0= \hat{g_j}(x) \times 0= \hat{g_j}(x)$. This shows that $\hat{h}$ has continuous behavior between transitioning from case to case of its output. Further, when $d(x) \neq 0, \epsilon$, then $\hat{h}$ is continuous since $g$ is continuous as required, and thus $\hat{g_i}$ are continuous $\forall i$, as well as $\hat{g_i}\times \frac{2d(x)}{\epsilon}$, as the multiplied expression is simply a constant.    
\end{proof}


% \begin{proposition}
% Given a binary classification model $h: R^n \rightarrow \{0,1\}$, and a constant $\epsilon < 0$, it is possible to construct a model $\hat{h}$ with arbitrary gradients everywhere except within $\epsilon$ of a decision boundary, but maintains the same mapping $\hat{h}: R^n \rightarrow \{0,1\} = h: R^n \rightarrow \{0,1\}$. Specifically, this means that $h$ and $\hat{h}$ will have the same 0/1 loss, but arbitrarily different gradient-based explanations. 
% \end{proposition}
% \begin{proof}
% We divide the 
% Suppose we are given $g$

% \end{proof}

% \begin{proposition}
% Consider a binary classfication model $h: R^n \rightarrow [0,1]$, whose outputs we threshold to determine a mapping $h: R^n \rightarrow \{0,1\}$. We can create a model $\hat{h}$ with arbitrary explanations, but maintains the same mapping from 
% \end{proposition}
% \begin{proof}

% \end{proof}

==> questions.tex <==
Questions:

02 Background:
- Is my motivation ok of why we don't consider other approaches? Feel like it's a little rough.
- Within this specification, we evaluate our results on methods that return only one counterfactual point, can produce counterfactuals on deep models, and have open-source implementations freely available. Do we still want these further specifications?

-Interestingly, Theorem~\ref{theorem:loss-and-lipschitz} also explains why counterfactuals with high cost, even if they are relatively from the decision boundary, may not ensure high consistency in deep models, as we saw in Figure~\ref{fig:toy-non-linear}. The counterfactual with high confidence may sit in a region with high local Lipschitz Constant; therefore, the magnitude of gradient signal in minimizing the Cross Entropy may be strong enough to cause the point to change prediction in a nearby model. Is this true? (End of section 4.1)

==> related_work.tex <==
% !TEX ROOT=./neurips_2021.tex
\paragraph{Counterfactual Explanations.} A counterfactual explanation for a given point is a nearby point that receives the different, often specified, prediction from a model: for example, a counterfactual explanation for a rejected loan application is a nearby hypothetical application that was accepted. Formally, a counterfactual example on a point $x$,  in a model $f$, for desired outcome $c$, is defined as $x_c= \text{argmin}_{x_c | f(x_c)=c} |x-x_c|_p$, where $p$ denotes the desired norm. 

%Counterfactual explanations are a method to either understand a model's decision on a given point, or provide clues for how an individual subject to a model's decision may change their behavior (and thus their input to the model) to get a different result, i.e. to provide recourse. 
The \emph{cost} of a counterfactual is its distance from the original point, i.e. $|x-x_c|_p$. Common desiderata in generating counterfactuals are low-cost (for attainability in the recourse setting), sparsity (for ease of understanding), causal motivation ~\cite{}, and realism, i.e. being within the data distribution. While there are several methods of generating counterfactuals that trade off between these desiderata~\cite{}, we restrict our investigation to methods that can be used on deep models, and within this, two main types: generation methods that endeavor to find the \emph{nearest} point to the input point requiring an explanation, i.e. of lowest cost, first introduced by Wachter et al.~\cite{wachter2018counterfactual}, and generation methods that sacrifice counterfactual cost in order to have a nearby point that is in the data manifold~\cite{pawelczyk,everyoneelse}. %This decision is in keeping with prior work in the area.


%The seminal work on counterfactual explanations was introduced by Wachter et. al.~\citep{wachter2018counterfactual}

\paragraph{Counterfactual Consistency and Invalidation.} Recent work by Pawelczyk et al. has also investigated the consistency of counterfactual examples across similar models, although they restrict their analysis to highly callibrated models, and experimentation to linear and random forest models~\cite{}. They, along with other work that investigates counterfactual inconsistency across large scale distribution shifts~\cite{rawal2021i}, show that higher-cost counterfactuals are less likely to be invalidated than lower-cost counterfactuals in linear, or well-calibrated models. In this paper, we focus on evaluating the problem of counterfactual inconsistency in deep models, where this assumption of calibraton does not hold. Further, unlike prior work, we introduce a method to mitigate counterfactual inconsistency in deep models that reaches low invalidation while keeping a relatively low cost.

We follow Pawelczyk et al.'s definition of a consistency metric for counterfactual examples across models: the \emph{invalidation rate}. A counterfactual example $x_c$ generated in some model $F$ is \emph{invalidated} in a model $F'$ if $F(x_c)\neq F'(x_c)$. Throughout this paper, we will call the model $F$that creates the counterfactual the \emph{generating} model. 

\paragraph{Model Duplicity.}
%Recent work has shown that duplicitious models,
In this work, we demonstrate and address the problem of deep models with arbitrary differences producing varying outputs on \emph{counterfactual explanations}. Recent work has shown that there are large differences between model prediction behavior on ~\emph{any} input across small changes to the model, not specifically counterfactual examples~\cite{blackleave2021,}. We, along with Marx et al. (and Pawelczyk et al.)~\cite{flavio}, restrict the models we evaluate consistency over to be within a certain accuracy bound of a trained baseline model. However, unlike Marx et al. and Pawelczyk et al, we only consider changes to the model that are "arbitrary" in that they do not affect the model's optimization function. Specifically, we restrict our search of nearby models to those only differing in the random initialization and small changes to the training set, instead of searching over hyperparameters.


%\paragraph{Broader Notions of Explanation Instability.} Other works investigating instability of explanation techniques in deep models focus on the instability of gradient-based approaches across very similar \emph{inputs}, i.e. adversarially perturbing an input to a model to receive a very different explanation for a similar input~\cite{}. There are also some works that develop adversarial attacks to create similar models that have differing gradient-based explanations~\cite{fairwashing}. Contrastingly, this work focuses on the instability of counterfactual explanations between similar models, e.g. those created throughout deployment, outside of an adversarial context.



% We restrict these differences to be small, arbitrary ones that may occur as updates during model deployment, such as a change in random seed or a small change in training set,  

% We are motivated by the setting of models used during deployment . 

% Inconsistencies between similar models do not stop at explanations, but extend into model predictions themselves: recent work has shown that duplicitious models, i.e. models with very similar accuracy, can often have large differences in individual-level prediction behavior. That is, a substantial portion of individuals who are subject to decisions from a model may have their decisions changed as a result of  differences that do not affect accuracy in aggregate~\cite{blackleave2021,marx2019}. This behavior has been shown to be most prevalent in deep models, and can even occur as the result of completely arbitrary differences such as a one-point differences in the training set, or random initialization~\cite{blackleave2021}. 

% \paragraph{Consistency in Predictions and Explanations.} There is growing work drawing attention to the instability of various explanation methods, both for counterfactual and other explanation approaches. Previous work has investigated the problem of counterfactual invalidation between duplicitious linear and random forest models~\cite{}, and also in a variety of models in response to large-scale distribution shift (e.g. retraining on a related but different dataset)~\cite{}. Both of these papers find that there is a trade-off between the cost of counterfactual examples, i.e. the distance between the original point in question and its counterfactual, and the chance that it will be invalidated in a new model. Specifically, they show that higher-cost counterfactuals are less likely to be invalidated than lower-cost counterfactuals. It remains untested to what extent this intuition holds in deep models, which is part of what we address in this paper. We find that this intuition does not always hold---sometimes increasing counterfactual cost does not lead to decreased invalidation in deep models---but we also find that there is a relatively low-cost methods of generating stable counterfactuals, namely robust neighbor search (RNS).

% %This work focuses on the instability of counterfactual explanations between similar models, 
% %Although this is the first work investigating 
% Other works investigating instability of explanation techniques in deep models focus on the instability of gradient-based approaches across very similar \emph{inputs}, i.e. adversarially perturbing an input to a model to receive a very different explanation for a similar input~\cite{}. There are also some works that develop adversarial attacks to create similar models that have differing gradient-based explanations~\cite{fairwashing}. Contrastingly, this work focuses on the instability of counterfactual explanations between similar models, outside of an adversarial context.

% \paragraph{Model Duplicity.}
% %Recent work has shown that duplicitious models,
% Stability problems between similar models do not stop at explanations, but extend into model predictions themselves: recent work has shown that duplicitious models, i.e. models with very similar accuracy, can often have large differences in individual-level prediction behavior. That is, a substantial portion of individuals who are subject to decisions from a model may have their decisions changed as a result of  differences that do not affect accuracy in aggregate~\cite{blackleave2021,marx2019}. This behavior has been shown to be most prevalent in deep models, and can even occur as the result of completely arbitrary differences such as a one-point differences in the training set, or random initialization~\cite{blackleave2021}. 

==> scrap.tex <==
Even further, as we see from the counterfactuals generated for point $x_2$ in Figure ~\ref{fig:toy-non-linear}, comparing the decision surfaces of two DNNs trained on the same synthetic dataset pictured, where the grey shaded regions denote where one model predicts the blue class, the darker grey shaded regions show where the other model predicts the blue class, and the black areas are where the decision surfaces overlap.  even We demonstrate that there is no strong correlation between cost and invalidation percentage on real datasets in Section ~\ref{sec:evaluation}, by showing that counterfactuals with higher costs may have higher invalidation rates than counterfactuals with lower cost~\ref{table:results}, and that the $R^2$ coefficient between counterfactual cost and invalidation is \emily{TODO:fill in.}

\begin{Lemma}\label{lemma:deep_boundaries}
%Consider a deep model $F(\theta, \xvec)$ with 
In deep models, a higher distance from the \emph{closest} boundary does not guarantee being far away from \emph{any} boundary.
\end{Lemma}
\begin{proof}
We prove this lemma by demonstration. Consider Figure ~\ref{fig:toy-non-linear}, which we created by training a DNN on the synthetic dataset pictured in Figure ~\ref{fig:toy-dataset}. The grey shaded regions denote where the model predicts the blue class. See that for point $x_1$, the higher-cost counterfactual generated for that point in the is actually closer to a decision boundary than the lower-cost counterfactual.
\end{proof}
Thus, cost is not a reliable metric to determine counterfactual stability at generation time: a counterfactual example with a higher cost, while perhaps further from the nearest boundary to the origin point, may in fact be closer to some boundary $b'$, making its prediction potentially equally or even more sensitive to small perturbations to the decision surface. 

Even further, as we see from the counterfactuals generated for point $x_2$ in Figure ~\ref{fig:toy-non-linear}, even We demonstrate that there is no strong correlation between cost and invalidation percentage on real datasets in Section ~\ref{sec:evaluation}, by showing that counterfactuals with higher costs may have higher invalidation rates than counterfactuals with lower cost~\ref{table:results}, and that the $R^2$ coefficient between counterfactual cost and invalidation is \emily{TODO:fill in.}
%it highly likely to be invalidated
, and the darker grey shaded regions show where the other model predicts the blue class.The black areas are where the decision surfaces overlap.

==> table_redone.tex <==
\begin{table}[t]
\resizebox{\textwidth}{!}{%
    \begin{tabular}{c|cc|cc|cc|cc|cc|cc}
        \multicolumn{13}{c}{Invalidation Rate  (Leave-One-Out, Random Seed)} \\
        \toprule 
        \textbf{Approach}&\multicolumn{2}{c}{German Credit} & \multicolumn{2}{c}{Seizure} & \multicolumn{2}{c}{CTG} & \multicolumn{2}{c}{Warfarin}&\multicolumn{2}{c}{HELOC}& \multicolumn{2}{c}{Taiwanese Credit}\\
        \textbf&LOO & RS & LOO  & RS&LOO& RS&LOO & RS & LOO  & RS&LOO & RS \\
        \midrule
        \rowcolor{black!5} Wachter et al. &  &  &  & & &  &  &  &  & & & \\
        \rowcolor{black!5} Min. $\epsilon$ PGD & 0.28 &  0.61 & 0.94 & 0.94& 0.02& 0.11 &0.10& 0.12& 0.04 & 0.11 &0.04 & 0.24\\
        $\quad \quad$+RNS & \textbf{0.00} & 0.13 &0.03 & 0.15 & \textbf{0.00} & \textbf{0.00} &0.01& 0.02& 0.00&  \textbf{0.00} &\textbf{0.00} & 0.11\\
        \rowcolor{black!5} CW & 0.39 & 0.55 & 0.68&0.83& -&-& && 0.01&0.05 &0.07&0.19\\
        $\quad \quad$+RNS & 0.01 & \textbf{0.05} & \textbf{0.02} & 0.13& - &-& &&0.00&\textbf{0.00}&\textbf{0.00}&\textbf{0.01}\\
        \rowcolor{black!5} Pawelczyk et al. & 0.2 &0.35 &0.16 &\textbf{0.12} && &0.02&0.01& 0.04& 0.05& 0.01 &0.20\\
        \rowcolor{black!5} Looveren et al. &  &  &  & & & &  &  &  & & & \\

        % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
        % \rowcolor{black!5} \textsuperscript{16}O & 0 & 99.96 & -&& &\\
        % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
        \bottomrule
        % \\
        % \multicolumn{7}{c}{Invalidation Rate (Random Seed)} \\
        % \toprule 
        % \textbf{Approach}&German Credit & Seizure & CTG  & Warfarin&HELOC& Taiwanese Credit\\
        % \midrule
        % \rowcolor{black!5} Wachter et al. &  &  &  & & & \\
        % \rowcolor{black!5} Min. $\epsilon$ PGD & 0.61 & 0.94 &0.11 &0.12& 0.11&0.24\\
        % $\quad \quad$+RNS & 0.13 & 0.15& \textbf{0.00}&0.02&\textbf{0.00}& 0.11\\
        % \rowcolor{black!5} CW & 0.55 &0.83  & -&&0.05 &0.19\\
        % $\quad \quad$+RNS & \textbf{0.05} &  0.13& -&&\textbf{0.00}&\textbf{0.01}\\
        % \rowcolor{black!5} Pawelczyk et al. & 0.35 & \textbf{0.12}& &0.01&0.05 &0.20\\
        % \rowcolor{black!5} Looveren et al. &  &  &  & & & \\
        % % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
        % % \rowcolor{black!5} \textsuperscript{16}O & 0 & 99.96 & -&& &\\
        % % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
        % \bottomrule
        % \\
        % \multicolumn{7}{c}{Cost of Counterfactual Explanations} \\
        % \toprule 
        % \textbf{Approach}&German Credit & Seizure & CTG & Warfarin&HELOC& Taiwanese Credit\\
        % \midrule
        % Min. $\epsilon$ PGD &  & & &&& \\
        % % \rowcolor{black!5} CW &  &  & && &\\
        % CW &  &  &  & & &\\
        % % \rowcolor{black!5} PGDs &  && && &\\
        % PGD+RNS &3.01 &6.10 & &0.50&1.79&\textbf{2.78} \\
        % % \rowcolor{black!5} CW &  &  & && &\\
        % CW+RNS & \textbf{2.63} & \textbf{6.01} &  &&1.75&3.37\\
        % \rowcolor{black!5} AE &7.15  &13.7 &&2.62& \textbf{1.35}&4.24\\
        % \rowcolor{black!5} Looveren et al. &  &  &  & & & \\

        % % \textsuperscript{15}N & \sfrac{1}{2} & 0.40 & 30.2 &&&\\
        % % \rowcolor{black!5} \textsuperscript{16}O & 0 & 99.96 & -&& &\\
        % % \textsuperscript{17}O & \sfrac{1}{2} & 0.04 & 40.4&&& \\
        % \bottomrule
        % \\
    \end{tabular}%
    }
    \caption{Invalidation Rate ... TODO}
    \end{table}
    \label{table_IV}
